A Short Course on Frame Theory

A Short Course on Frame Theory.

==> frames-ieee 2/acronyms_list_frames.tex <==
% Frames's Acronyms
%\begin{acronym}
\acrodef{ONB}[ONB]{orthonormal basis}%{=description}%{=orthonormal basis}%{=description}
\acrodef{ada}[A/D]{analog-to-digital}%{=description}%{=orthonormal basis}%{=description}
\acrodef{daa}[D/A]{digital-to-analog}%{=description}%{=orthonormal basis}%{=description}
\acrodef{dfta}[DFT]{discrete Fourier transform}%{=description}%{=orthonormal basis}%{=description}
\acrodef{dtfta}[DTFT]{discrete-time Fourier transform}%{=description}%{=orthonormal basis}%{=description}
\acrodef{cdmaa}[CDMA]{code division multiple access}%{=description}%{=orthonormal basis}%{=description}
\acrodef{ofdma}[OFDM]{orthogonal frequency division multiplexing}%{=description}%{=orthonormal basis}%{=description}
\acrodef{wha}[WH]{Weyl-Heisenberg}%{=description}%{=orthonormal basis}%{=description}
%\end{acronym}

% \newacronym{ONB}{orthonormal basis}{=description}%{=orthonormal basis}%{=description}
% \newacronym[ada]{A/D}{analog-to-digital}{=description}%{=orthonormal basis}%{=description}
% \newacronym[daa]{D/A}{digital-to-analog}{=description}%{=orthonormal basis}%{=description}
% \newacronym[dfta]{DFT}{discrete Fourier transform}{=description}%{=orthonormal basis}%{=description}
% \newacronym[dtfta]{DTFT}{discrete-time Fourier transform}{=description}%{=orthonormal basis}%{=description}
% \newacronym[cdmaa]{CDMA}{code division multiple access}{=description}%{=orthonormal basis}%{=description}
% \newacronym[ofdma]{OFDM}{orthogonal frequency division multiplexing}{=description}%{=orthonormal basis}%{=description}
% \newacronym[wha]{WH}{Weyl-Heisenberg}{=description}%{=orthonormal basis}%{=description}


% \newacronym[onba]{ONB}{orthonormal basis}{name=orthonormal basis (ONB)}%{=orthonormal basis}%{=description}
% \newacronym[ada]{A/D}{analog-to-digital}{name=analog-to-digital (A/D)}%{=orthonormal basis}%{=description}
% \newacronym[daa]{D/A}{digital-to-analog}{name=digital-to-analog (D/A)}%{=orthonormal basis}%{=description}
% \newacronym[dfta]{DFT}{Discrete Fourier Transform}{name=Discrete Fourier Transform (DFT)}%{=orthonormal basis}%{=description}
% \newacronym[dtfta]{DTFT}{Discrete-Time Fourier Transform}{name=Discrete-Time Fourier Transform (DTFT)}%{=orthonormal basis}%{=description}
% \newacronym[cdmaa]{CDMA}{code division multiple access}{name=code division multiple access (CDMA)}%{=orthonormal basis}%{=description}
% \newacronym[ofdma]{OFDM}{orthogonal frequency division multiplexing}{name=orthogonal frequency division multiplexing (OFDM)}%{=orthonormal basis}%{=description}
% \newacronym[wha]{WH}{Weyl-Heisenberg}{name=Weyl-Heisenberg (WH)}%{=orthonormal basis}%{=description}

% \chapter{Acronyms}
% 
% % tighter spacing of the acronym list
% \makeatletter
% \renewcommand{\bflabel}[1]{#1\hfill}
% \renewenvironment{AC@deflist}[1]%
% {\raggedright\begin{list}{}%
%        {\settowidth{\labelwidth}{\textbf{\textsf{#1}}}%
%         \setlength{\leftmargin}{\labelwidth}%
%         \addtolength{\leftmargin}{\labelsep}%
%         \setlength{\itemsep}{0ex}%
%         \setlength{\parsep}{0ex}%
%         \renewcommand{\makelabel}{\bflabel}}%
% }%
% {\end{list}%
% }%
% \makeatother
% 
% \begin{acronym}
% \acro{onba}[ONB]{orthonormal basis}%{name=orthonormal basis (ONB)}%{=orthonormal basis}%{=description}
% \acro{ada}[A/D]{analog-to-digital}%{name=analog-to-digital (A/D)}%{=orthonormal basis}%{=description}
% \acro{daa}[D/A]{digital-to-analog}%{name=digital-to-analog (D/A)}%{=orthonormal basis}%{=description}
% \acro{dfta}[DFT]{Discrete Fourier Transform}%{name=Discrete Fourier Transform (DFT)}%{=orthonormal basis}%{=description}
% \acro{dtfta}[DTFT]{Discrete-Time Fourier Transform}%{name=Discrete-Time Fourier Transform (DTFT)}%{=orthonormal basis}%{=description}
% \acro{cdmaa}[CDMA]{code division multiple access}%{name=code division multiple access (CDMA)}%{=orthonormal basis}%{=description}
% \acro{ofdma}[OFDM]{orthogonal frequency division multiplexing}%{name=orthogonal frequency division multiplexing (OFDM)}%{=orthonormal basis}%{=description}
% \acro{wha}[WH]{Weyl-Heisenberg}%{name=Weyl-Heisenberg (WH)}%{=orthonormal basis}%{=description}
% \end{acronym}

\newcommand{\onbac}{\ac{ONB}\xspace}
\newcommand{\onbacp}{\acp{ONB}\xspace}
\newcommand{\adac}{\ac{ada}\xspace}
\newcommand{\daac}{\ac{daa}\xspace}
\newcommand{\dftac}{\ac{dfta}\xspace}
\newcommand{\dtftac}{\ac{dtfta}\xspace}
\newcommand{\dtftacp}{\acp{dtfta}\xspace}
\newcommand{\cdmaac}{\ac{cdmaa}\xspace}
\newcommand{\ofdmac}{\ac{ofdma}\xspace}
\newcommand{\whac}{\ac{wha}\xspace}

% \newcommand{\onbac}{\onba\xspace}
% \newcommand{\adac}{\ada\xspace}
% \newcommand{\daac}{\daa\xspace}
% \newcommand{\dftac}{\dfta\xspace}
% \newcommand{\dtftac}{\dtfta\xspace}
% \newcommand{\cdmaac}{\cdmaa\xspace}
% \newcommand{\ofdmac}{\ofdma\xspace}
% \newcommand{\whac}{\wha\xspace}

==> frames-ieee 2/book-macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LaTeX PACKAGE INCLUSION %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage[cm]{fullpage}

% \usepackage{babel}
\usepackage{paralist}
\usepackage{array}
%\usepackage{multirow}
%\usepackage{booktabs}
\usepackage{cite}
\usepackage{graphics}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{units}
\usepackage{cases}
\usepackage{subfigure}
\usepackage{hyperref}
%\usepackage[acronym=true,toc=true,number=none,style=long,border=none,header=none,cols=2]{packages/glossary}
\usepackage{makeidx}


% \hypersetup{
% pdfauthor = {Erchin SERPEDIN and Serhan YARKAN},
% pdftitle = {Signal Processing},
% pdfsubject = {Textbook, 2010},
% pdfkeywords = {mathematics, signal processing},
% pdfcreator = {\LaTeX},
% pdfproducer = {Serhan YARKAN}
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LaTeX PACKAGE INCLUSION - END %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%% ACRONYM-RELATED MACROS %%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newcommand{\ac}{\useacronym}
% \newcommand{\Ac}{\ac}
% 
% \newcommand{\acp}{\useacronym[s]}
% \newcommand{\Acp}{\acp}
% 
% \newcommand{\acl}{\acrln}
% \newcommand{\Acl}{\acl}
% 
% \newcommand{\acs}{\acrsh}
% \newcommand{\Acs}{\acs}
% 
% \newcommand{\acc}{\useacronym*}
% \newcommand{\Acc}{\acc}
% 
% \newcommand{\accp}{\useacronym*[s]}
% \newcommand{\Accp}{\accp}
% 
% \newcommand{\accl}{\acrln*}
% \newcommand{\Accl}{\accl}
% 
% \newcommand{\acclp}[1]{\acl{#1}{s}}
% \newcommand{\Acclp}{\acclp}
% 
% 
% \makeacronym
% \setacronymnamefmt{\gloshort}
% \setacronymdescfmt{\glolong}
% \renewcommand\gloskip{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% ACRONYM-RELATED MACROS-END  %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% FOOTNOTE LABELING AND REFERENCING %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def \footnotelabel{%
\edef\@currentlabel{\p@footnote\thefootnote}%
\label} \makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% FOOTNOTE LABELING AND REFERENCING - END %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% LaTeX COMPILING MODE SELECTION %%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \ifx\pdfoutput\undefined
% % we are running LaTeX, not pdflatex
% \usepackage{graphicx}
% \else
% % we are running pdflatex, so convert .eps files to .pdf
% \usepackage[pdftex]{graphicx}
% \usepackage{epstopdf}
% \fi 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% LaTeX COMPILING MODE SELECTION - END %%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% COMPACT REFERENCING SETTINGS %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\citepunct{, }
\renewcommand\citedash{--}
\newcommand{\Chref}[1]{Chapter~\ref{#1}}
\newcommand{\Secref}[1]{Section~\ref{#1}}
\newcommand{\Figref}[1]{Figure~\ref{#1}}
\newcommand{\Tblref}[1]{Table~\ref{#1}}
\newcommand{\Ftref}[1]{Footnote~\ref{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% COMPACT REFERENCING SETTINGS - END %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \makeindex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MATHEMATICAL OPERATOR DECLARATION MACRO %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\DMO}[1]{\expandafter\DeclareMathOperator*{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MATHEMATICAL OPERATOR DECLARATION MACRO -END %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% LIST OF SYMBOLS CONSTRUCTION MACRO %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\listofsymbols{\input{notation_and_symbols} \clearpage}
\def\addsymbol #1: #2#3{$#1$ \> \parbox{5in}{#2 \dotfill \pageref{#3}}\\}
\def\defsym#1{\label{#1}} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% LIST OF SYMBOLS CONSTRUCTION MACRO - END %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SHORTHANDS FOR FREQUENTLY USED ITEMS %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\qmark}[1]{``#1''} % Place quotation marks around its input
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SHORTHANDS FOR FREQUENTLY USED ITEMS - END %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Left numbered bullet style definition
\newcounter{ADD}
\def\additionletter{A}
\newcommand{\cntRm}[1]{\stepcounter{#1}\Roman{#1}}
\newcommand{\cntAr}[1]{\stepcounter{#1}\arabic{#1}}
\newcommand{\cntAl}[1]{\stepcounter{#1}\alph{#1}}
\newcommand{\addit}{\mathcal{\expandafter\uppercase\expandafter{\additionletter}}}
\newcommand{\itemizeinput}{\bullet}


\def\normletter{N}
\newcommand{\normit}{\mathcal{\expandafter\uppercase\expandafter{\normletter}}}

\newcommand{\addbulletR}[1]{\ensuremath{\mathbf{(#1.\cntRm{ADD})}}~}
\newcommand{\addbulletAr}[1]{\ensuremath{\mathbf{(#1.\cntAr{ADD})}}~}
\newcommand{\addbulletAl}[1]{\ensuremath{\mathbf{(#1.\cntAl{ADD})}}~}

\newcommand{\newbullet}[3]{\ensuremath{\mathbf{#2#1#3}}~}

\newcommand{\newbulletPP}[1]{\ensuremath{\mathbf{(#1)}}~}
\newcommand{\nwbllt}[1]{\newbullet{#1}{}{}}% Left numbered bullet style definition

\newcommand{\PP}[1]{\left(#1\right)} % Parantheses
\newcommand{\CJ}[1]{#1^{*}} % Complex conjugation

\newcommand{\DLM}[3]{\ensuremath{\left\expandafter#1#2\right\expandafter#3}}

\newcommand{\set}[1]{\ensuremath{\left\{#1\right\}}} % Set
\newcommand{\Set}{\set} % Set (ALIAS)

\newcommand{\F}[1]{\ensuremath{\pmb{\mathcal{#1}}}} % Field

\newcommand{\EX}[1]{\ensuremath{\setminus\{#1\}}} % Except (set difference)

\newcommand{\Exists}{\exists} % There exists (ALIAS)

\newcommand{\existsonlyone}{\exists!} % There exist only one
\newcommand{\Existsonlyone}{\existsonlyone} % There exist only one (ALIAS)

\newcommand{\VS}[1]{\ensuremath{\mathfrak{#1}}} % Vector Space
\newcommand{\V}[1]{\ensuremath{\expandafter\lowercase\expandafter{\mathbf{#1}}}} % Vector

\newcommand{\AND}[2]{#1\wedge #2}


\DMO{\linearspan}{span} % Linear span
\newcommand{\Span}[1]{\linearspan\PP{#1}}% Linear span MACRO

\newcommand{\Dim}[1]{\dim\PP{#1}}% Dimension
\newcommand{\Real}[1]{\mathbb{R}^{#1}}
\newcommand{\Nature}{\mathbb{N}}

\newcommand{\M}[1]{\ensuremath{\expandafter\uppercase\expandafter{\mathbf{#1}}}} % Matrix
\newcommand{\norm}[1]{\ensuremath{\left\lVert#1\right\rVert}} % Norm
\newcommand{\Norm}{\norm} % Norm (ALIAS)

\newcommand{\abs}[1]{\ensuremath{\left\vert#1\right\vert}} % Absolute value
\newcommand{\Abs}{\abs} % Absolute value (ALIAS)

\newcommand{\MS}[1]{\ensuremath{\mathsf{#1}}} % Metric space
\newcommand{\INP}[2]{\ensuremath{\left\langle#1\mid#2\right\rangle}} % Inner product
\newcommand{\Herm}[1]{\ensuremath{#1^{\dag}}} % Hermitian transpose

\DeclareMathOperator*{\range}{\mathcal{R}} % Range (in linear algebra) operator
\newcommand{\Range}[1]{\ensuremath{\range\PP{#1}}} % Range MACRO

\DeclareMathOperator*{\image}{\mathcal{I}m} % Range (in linear algebra) operator
\newcommand{\Image}[1]{\ensuremath{\image\PP{#1}}} % Image MACRO

\DeclareMathOperator*{\kernel}{\mathcal{K}er} % Kernel (in linear algebra) operator
\newcommand{\Kernel}[1]{\ensuremath{\kernel\PP{#1}}} % Kernel MACRO

\DeclareMathOperator*{\nullity}{\mathcal{N}ull} % Nullity (in linear algebra) operator
\newcommand{\Nullity}[1]{\ensuremath{\nullity\PP{#1}}} % Nullity MACRO

\DeclareMathOperator*{\rank}{rank} % Rank operator
\newcommand{\Rank}[1]{\ensuremath{\rank\PP{#1}}} % Rank MACRO

\DeclareMathOperator*{\rowrank}{row\rank} % Row-Rank operator
\newcommand{\rowRank}[1]{\ensuremath{\rowrank\PP{#1}}} % Row-Rank MACRO
\newcommand{\RowRank}{\rowRank} % Row-Rank MACRO (ALIAS)

\DeclareMathOperator*{\colrank}{column\rank} % Column-Rank operator
\newcommand{\colRank}[1]{\ensuremath{\colrank\PP{#1}}} % Column-Rank MACRO
\newcommand{\ColRank}{\colRank} % Column-Rank MACRO (ALIAS)

\DeclareMathOperator*{\adjoint}{adj} % Adjoint operator
\newcommand{\adj}[1]{\ensuremath{\adjoint\PP{#1}}} % Adjoint operator MACRO
\newcommand{\Adj}{\adj} % Adjoint operator MACRO (ALIAS)

\DeclareMathOperator*{\trace}{tr} % Trace operator
\newcommand{\tr}[1]{\ensuremath{\trace\PP{#1}}} % Trace operator MACRO
\newcommand{\Tr}{\tr} % Trace operator MACRO (ALIAS)

\DeclareMathOperator*{\diagonal}{diag} % Diagonal operator
\newcommand{\diag}[1]{\ensuremath{\diagonal\PP{#1}}} % Diagonal MACRO
\newcommand{\Diag}{\diag} % Diagonal MACRO (ALIAS)


\DeclareMathOperator*{\condition}{cond} % Condition number operator
\newcommand{\cond}[1]{\condition\PP{#1}} % Condition number operator MACRO
\newcommand{\Cond}{\cond} % Condition number operator MACRO (ALIAS)



\newcommand{\rv}[1]{\mathcal{#1}} % Random variable MACRO
\newcommand{\Rv}{\rv} % Random variable MACRO (ALIAS)
\newcommand{\RV}{\rv} % Random variable MACRO (ALIAS)

\newcommand{\pr}[1]{\Pr\PP{#1}} % Probability MACRO
\newcommand{\PR}{\pr} % Probability MACRO (ALIAS)

%\newcommand{\std}[1]{\stdeviation\PP{#1}} % Standard deviation operator MACRO
%\newcommand{\Std}{\std} % Standard deviation operator MACRO (ALIAS)

\DeclareMathOperator*{\mn}{mean} % Mean operator
\newcommand{\mean}[1]{\ensuremath{\mn\PP{#1}}} % Mean operator MACRO
\newcommand{\Mean}{\ensuremath{\mean}} % Mean operator MACRO (ALIAS)
\newcommand{\MEAN}[1]{\ensuremath{\mu_{#1}}} % Mean operator (mu) MACRO (ALIAS)
\newcommand{\MEANBAR}[1]{\ensuremath{\overline{#1}}} % Mean operator (mu) MACRO (ALIAS)

\DeclareMathOperator*{\stdeviation}{std} % Standard deviation operator
\newcommand{\std}[1]{\ensuremath{\stdeviation\PP{#1}}} % Standard deviation operator MACRO
\newcommand{\Std}{\ensuremath{\std}} % Standard deviation operator MACRO (ALIAS)
\newcommand{\STD}[1]{\ensuremath{\sigma_{#1}}} % Standard deviation (sigma) operator MACRO (ALIAS)

\DeclareMathOperator*{\variance}{var} % Variance operator
\newcommand{\var}[1]{\ensuremath{\variance\PP{#1}}} % Variance operator MACRO (ALIAS)
\newcommand{\Var}{\ensuremath{\var}} % Variance operator MACRO (ALIAS)
\newcommand{\VAR}[1]{\ensuremath{\sigma_{#1}^{2}}} % Variance (sigma-squared) operator MACRO (ALIAS)

\newcommand{\ev}[1]{\ensuremath{E\Set{#1}}} % Expected value operator MACRO
\newcommand{\EV}{\ev} % Expected value operator MACRO (ALIAS)











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% [amsmath] ENVIRONMENT SETTINGS %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% modified for Frames chapter
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}

\theoremstyle{definition}
\newtheorem{dfn}[thm]{Definition}
\newtheorem{xca}[thm]{Exercise}
\newtheorem{example}[thm]{Example}
	
	% \newtheorem{rem}{Remark}
	
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% [amsmath] ENVIRONMENT SETTINGS - END %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> frames-ieee 2/defs.tex <==
%!TEX root = ncblock.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% defs.tex
% 
% Veniamin Morgenshtern 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%: frame theory
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\safemath{\vsignal}{\vecx}				% signal in finite-dimensions
\safemath{\altvsignal}{\vecy}			% alternative signal in finite-dimensions
\safemath{\csignal}{\fun}				% continous signal
\safemath{\altcsignal}{\altfun}			% continous signal
\safemath{\analop}{\opT}				% analysis operator
\safemath{\lianalop}{\opL}				% analysis operator
\safemath{\dualanalop}{\tilde\opT}				% analysis operator
\safemath{\manalop}{\matT}				% analysis operator finite dimension
\safemath{\analcrossop}{{\opT^{\times}}}			% what will become adjoint to analysis operator
\safemath{\synthdualop}{\ad{\tilde\opT}}		% synthesis operator with dual functions
\safemath{\msynthdualop}{\tp{\tilde\matT}}		% matrix representing synthesis operator with dual functions
\safemath{\msynthdualopc}{\herm{\tilde\matT}}		% matrix representing synthesis operator with dual functions, complex case
\safemath{\msynthop}{\tp{\matT}}		% matrix representing synthesis operator with dual functions
\safemath{\analdualop}{\tilde\opT}		% analysis operator with dual functions
\safemath{\vbasisel}{\vece}			% basis element in finite dimensions (for analysis)
\safemath{\vsynthbasisel}{\tilde\vece}	% basis element in finite dimensions (for synthesis)
\safemath{\synthbasisel}{\tilde e}	% basis element in infinite dimensions (for synthesis)
\safemath{\basisel}{e}	% basis element in infinite dimensions (for synthesis)
\safemath{\vanalframeel}{\vecg}			% frame element in finite dimensions (for analysis)
\safemath{\vanalframeelc}{g}			% component of frame element in finite dimensions (for analysis)
\safemath{\vsynthframeel}{\tilde\vecg}	% frame element in finite dimensions (for synthesis)
\safemath{\analframeel}{g}			% frame element in infinite dimensions (for analysis)
\safemath{\analframeelrev}{\tilde g}			% frame element in infinite dimensions (for analysis) reversed!
\safemath{\synthframeel}{\tilde g}	% frame element in infinite dimensions (for synthesis)
\safemath{\synthframeelrev}{g}	% frame element in infinite dimensions (for synthesis) reversed!
\safemath{\cframeel}{g}					% frame element in continous time
\safemath{\vcoef}{\vecc}				% vector of expansion coefficients
\safemath{\coeflt}{\{c_k\}_{k\in\frameset}}				% vector of expansion coefficients
\safemath{\coefaltlt}{\{a_k\}_{k\in\frameset}}				% vector of expansion coefficients
\safemath{\coef}{c}						% expansion coefficient
\safemath{\coefalt}{a}					% alternative expansion coefficient
\safemath{\dimension}{M}				% dimension of the vector space
\safemath{\framesize}{N}				% dimension of the vector space
\safemath{\frameset}{\setK}				% set of frame coefficient index
\safemath{\frameA}{A}					% lower frame constant 
\safemath{\frameB}{B}					% upper frame constant 
\safemath{\frameAdual}{\tilde A}					% lower frame constant 
\safemath{\frameBdual}{\tilde B}					% upper frame constant
\safemath{\frameop}{\opS}				% frame operator 
\safemath{\mframeop}{\matS}				% frame operator 
\safemath{\dualframeop}{\tilde\opS}				% frame operator 
\safemath{\dualframeoprev}{\opS}				% frame operator 
\safemath{\sinterval}{T}				% sampling interval
\safemath{\diractrain}{\dirac_T}        % dirac train
\safemath{\ftdiractrain}{\ft{\dirac}_T}        % dirac train
\safemath{\funsampled}{\fun_T}        	% sampled signal
\safemath{\ftfunsampled}{\ft{\fun}_T}        	% sampled signal
\safemath{\LPfiltert}{h_{\text{LP}}} % ideal low pass filter in time domain
\safemath{\arbfiltert}{h}				% arbitrary dual filter in time domain
\safemath{\outfiltert}{h_{\text{out}}} % out-of-band filter in time domain
\safemath{\outfilterf}{{\ft h}_{\text{out}}} % out-of-band filter in freq domain

\safemath{\LPfilterf}{\ft{h}_{\text{LP}}} % ideal low pass filter in frequency domain
\safemath{\cutoff}{f_c} 				% cut-off frequency of the ideal low pass filter
\safemath{\oversampling}{K} 			% oversampling factor
\safemath{\sqintspaceBL}{\hilfunspace(\bandwidth)} 	% space of square integrable functions bandlimited to B Hz
\safemath{\qnoise}{w} 					% quantization noise
\safemath{\qnoisevar}{\sigma^2} 					% variance of quantization noise
\safemath{\mseo}{\sigma^2_{\text{oversampling}}} 					% variance of quantization noise
\safemath{\msec}{\sigma^2_{\text{critical}}} 					% variance of quantization noise
\safemath{\mseb}{\sigma^2_{\text{basis}}} 					% variance of quantization noise
\safemath{\msef}{\sigma^2_{\text{frame}}} 					% variance of quantization noise
\safemath{\setframe}{\{\analframeel_k\in\hilspace\}_{k\in\frameset}} 					% frame set
\safemath{\setframem}{\{\analframeel_k\}_{k\in\frameset},\, \analframeel_k\in\hilspace,\, k\in\frameset,}					% modified frame set
\safemath{\setframemm}{\{\analframeel_k\}_{k\in\frameset}}					% modified frame set
\safemath{\setdualframe}{\{\synthframeel_k\in\hilspace\}_{k\in\frameset}} 					% dual frame set
\safemath{\setdualframemm}{\{\synthframeel_k\}_{k\in\frameset}} 					% dual frame set
\safemath{\setframerev}{\{\analframeelrev_k\in\hilspace\}_{k\in\frameset}} 					% frame set
\safemath{\setframerevmm}{\{\analframeelrev_k\}_{k\in\frameset}} 					% frame set
\safemath{\setdualframerev}{\{\synthframeelrev_k\in\hilspace\}_{k\in\frameset}} 					% dual frame set
\safemath{\setdualframerevmm}{\{\synthframeelrev_k\}_{k\in\frameset}} 					% dual frame set
\safemath{\weylop}{\opW}				% Weyl operator 
\safemath{\window}{g}				% Weyl operator 
\safemath{\waveop}{\opV}				% Weyl operator 
\safemath{\arb}{\mathrm{arb}}				% Weyl operator 





\newcommand{\ent}[1]{\ensuremath{\left[#1\right]}} % entry of a matrix or a vector
\newcommand{\allel}{\diamond}						%place-holder for "all elements in the set"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%: statistics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\specdensity}[1]{c_{#1}}			% generic spectral density
\newcommand{\specdensitymat}[1]{\matC_{#1}}	% generic multivariate spectral density

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%: time and frequency definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\let\time\undefined
%\safemath{\bandwidth}{W}		% bandwidth
\safemath{\duration}{D}			% duration
%\safemath{\time}{t}				% time				
%\safemath{\freq}{f}				% frequency
\safemath{\dtdf}{\dtime,\dfreq}  % discrete time and frequency shorthand
\safemath{\altdtdf}{\altdtime,\altdfreq}
%\safemath{\dtime}{k}				% discrete time		
%\safemath{\dfreq}{n}				% discrete frequency
\safemath{\altdtime}{l}				% alt. discrete time		
\safemath{\altdfreq}{m}				% alt. discrete frequency

\safemath{\dtimetilde}{\tilde{\dtime}}				% discrete time		
\safemath{\dfreqtilde}{\tilde{\dfreq}}				% discrete frequency
\safemath{\altdtimetilde}{\tilde{\altdtime}}				% alt. discrete time		
\safemath{\altdfreqtilde}{\tilde{\altdfreq}}				% alt. discrete frequency

%\safemath{\Ddtime}{\dtime}		% Delta discrete time
%\safemath{\Ddfreq}{\dfreq}		% Delta discrete frequency
%\safemath{\delay}{\tau}			%delay
%\safemath{\doppler}{\nu}			% doppler
\safemath{\maxDoppler}{\doppler_{0}}		% maximum Doppler spreadsc
\safemath{\altmaxDoppler}{\widetilde{\maxDoppler}}
\safemath{\maxDelay}{\delay_{0}}			% maximum delay spread
\safemath{\altmaxDelay}{\widetilde{\maxDelay}}
%\safemath{\spread}{\Delta_{\CHop}}		% channel spread
\safemath{\altspread}{\widetilde{\Delta}_{\CHop}}
\safemath{\tstep}{T}				% time slot length
\safemath{\fstep}{F}				% frequency slot length
\safemath{\alttstep}{\widetilde{\tstep}}				% time slot length
\safemath{\altfstep}{\widetilde{\fstep}}				% frequency slot length
\safemath{\tfstep}{\tstep\fstep}	% product of time and slot frequency slot
\safemath{\srtfstep}{\sqrt{\tfstep}}
\safemath{\fslots}{N}			% # slots in frequency
\safemath{\tslots}{K}			% # slots in time
\safemath{\tslotstot}{\widetilde{\tslots}}
\safemath{\fslotstot}{\widetilde{\fslots}}
\safemath{\tslotsguard}{K'}
\safemath{\tfslots}{\tslots\fslots}	% # total slots shorthand
\safemath{\tfsamples}{\dtime\tstep,\dfreq\fstep}	% shortcut for TF-sampling
\safemath{\WHset}{(\logon,\tstep,\fstep)}
\safemath{\WHsetsquare}{(\logon,\srtfstep,\srtfstep)}
\safemath{\spreadset}{\setD}
\safemath{\altspreadset}{\setE}
\safemath{\spreadsquareset}{\widetilde{\spreadset}}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %: Gabor analysis
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\safemath{\logon}{g}						% Gabor Logon (elementary function)
\safemath{\logonp}{\logon(\time)}
\safemath{\altlogon}{\widetilde{\logon}}						% alt Gabor Logon (elementary function)
\safemath{\altaltlogon}{e}
\safemath{\altlogonp}{\altlogon(\time)}
\safemath{\altaltlogonp}{\altaltlogon(\time)}
\safemath{\slogon}{\logon_{\dtime,\dfreq}}	% T-F shifted Gabor logon
\safemath{\slogonp}{\slogon(\time)}	% T-F shifted Gabor logon
\safemath{\slogonset}{\left\{\logon(\time-\dtime\srtfstep)\cex{\dfreq\srtfstep\time}\right\}}
\safemath{\eftime}{a_{0}}	% effective time extension of a signal
\safemath{\efband}{b_{0}} % effective bandwidth of a signal
\safemath{\logonf}{G} %Fourier transform of the logon signal
\safemath{\logonfp}{\logonf(\freq)}
\safemath{\logonalt}{f}
\safemath{\logonaltp}{\logonalt(\time)}
\safemath{\slogonct}{\logon_{(\alpha,\beta)}}
\safemath{\slogonctalt}{\logon_{(\alpha',\beta')}}
% % \safemath{\slogon}{\logon_{\dtime,\dfreq}}	% T-F shifted Gabor logon
\safemath{\af}{A}						% ambiguity function
\safemath{\afp}{\af_{\logon}(\doppler,\delay)}	% '' parametrized
\safemath{\setloc}{\setG}
\safemath{\setloclogon}{\widetilde{\setG}}
\safemath{\dertau}{b}
\safemath{\dernu}{a}
\safemath{\dertaup}{\dertau_{\dtdf}}
\safemath{\dernup}{\dernu_{\dtdf}}
% 
% \safemath{\const}{c}
\safemath{\constM}{c_{M}}
\safemath{\constm}{c_{m}}
% 
\safemath{\corr}{d}
\safemath{\corrmat}{\matD}




%%%%%%%%%%%%%%%
%: misc math
%%%%%%%%%%%%%%%
\safemath{\sumdtime}{\sum_{\dtime=-\infty}^{\infty}} % infinite sum in discrete time
\safemath{\sumdfreq}{\sum_{\dfreq=-\infty}^{\infty}} % infinite sum in discrete frequency

\safemath{\sumdtimelimited}{\sum_{\dtime=-\tslots}^{\tslots}} % infinite sum in discrete time
\safemath{\sumdfreqlimited}{\sum_{\dfreq=-\fslots}^{\fslots}} % infinite sum in discrete frequency

\safemath{\altsumdtimelimited}{\sum_{\altdtime=-\tslots}^{\tslots}} % infinite sum in discrete time
\safemath{\altsumdfreqlimited}{\sum_{\altdfreq=-\fslots}^{\fslots}} % infinite sum in discrete frequency


 %\renewcommand{\setminus}{\backslash}						% \setA - \setB
 \safemath{\limintime}{\lim_{\tslotstot\to\infty}}	% discrete-time limit
 %\safemath{\imat}{\matidentity}
 %\newcommand{\diag}[1]{\mathrm{diag}\lefto(#1\right)}	% diagonalization operator
 %\newcommand{\spreadint}[1]{\int_{\doppler}\int_{\delay} #1 d\delay d\doppler}
\newcommand{\spreadint}[1]{\iint_{\reals^2} #1 d\delay d\doppler}

\newcommand{\intspecparamin}[1]{\int_{\abs{\specparam}< \maxDoppler\tstep} #1 d\specparam}
\newcommand{\intspecparamout}[1]{\int_{\maxDoppler\tstep<\abs{\specparam}< 1/2} #1 d\specparam}					% index set
% \newcommand{\cex}[1]{e^{\iu2\pi #1}}				% positive complex exponential
% \newcommand{\cexn}[1]{e^{-\iu2\pi #1}}			% negative complex exponential
\safemath{\euler}{\gamma}	% Euler constant
\safemath{\intdiscrete}{\int_{-1/2}^{1/2}}
\safemath{\intdiscretetwod}{\intdiscrete\intdiscrete}
%\safemath{\hilfunspacep}{\hilfunspace(\reals)}	% Hilbert function space parametrized
\safemath{\hilfuntimeband}{\hilfunspace(\bandwidth,\duration,\spillover)}
\safemath{\spillover}{\eta}
\safemath{\hilfunband}{\hilfunspace(\bandwidth)}
\newcommand{\timetrunc}[1]{\mathbb{D}_{#1}}	%time-truncation operator
\newcommand{\timetruncfilter}[1]{p_{#1}}		% time-truncation filter
\safemath{\alttimetruncfilter}{p_{\duration+2\maxDelay}}		% time-truncation filter
\safemath{\timetruncfilterp}{\timetruncfilter(\time)}
%\newcommand{\freqtrunc}[1]{\mathbb{B}_{#1}}	%time-truncation operator
\newcommand{\freqtrunc}[1]{\mathbb{B}_{#1}}	%bandwidth-truncation operator
%\safemath{\freqtrunc}{\mathbb{B}_{\bandwidth}}	%bandwidth-truncation operator
\safemath{\onb}{\phi}
\safemath{\indexonb}{m}
\safemath{\numonb}{M}
\safemath{\onbp}{\onb_{\indexonb}(\time)}
\safemath{\funloc}{f}
\safemath{\funlocp}{\funloc(\dd)}
%\newcommand{\eigmax}[1]{\lambda_{\text{max}}\{#1\}}
\safemath{\ofun}{\phi}
\safemath{\altofun}{\ofun'}
\safemath{\oindex}{m}
\safemath{\ofunp}{\ofun_\oindex(\time)}
\safemath{\altofunp}{\altofun_\oindex(\time)}
\safemath{\onum}{M} 

\newcommand{\citepar}[1]{\hspace{-0.06mm}\cite{#1}}




==> frames-ieee 2/math-macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% standard-macros.tex
% 
% $Id: standard-macros.tex 2531 2009-02-22 16:02:51Z schuster $
%
% Commonly used LaTeX macros.
% 
% (c) 2002 by Moritz Borgmann
% major changes by Ulrich Schuster, 12/03-09/07
% Now works with and requires an additional macro file that defines the
% notation convention for random quantities, matrices, vectors, sets, etc.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage{amsmath}
%\usepackage{amssymb}
\usepackage{amsfonts}
%\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{xspace}
\usepackage{bm}
\usepackage{fancyref}
\usepackage{textcomp}
\usepackage[Symbol]{upgreek}

\newcommand{\safemath}[2]{\newcommand{#1}{\ensuremath{#2}\xspace}}

\newcommand{\erc}{\mathrm{ERC}}

%%%%% Sans Serif Math %%%%

% lower case
\newcommand{\ssa}{\mathsf{a}}
\newcommand{\ssb}{\mathsf{b}}
\newcommand{\ssc}{\mathsf{c}}
\newcommand{\ssd}{\mathsf{d}}
\newcommand{\sse}{\mathsf{e}}
\newcommand{\ssf}{\mathsf{f}}
\newcommand{\ssg}{\mathsf{g}}
\newcommand{\ssh}{\mathsf{h}}
\newcommand{\ssi}{\mathsf{i}}
\newcommand{\ssj}{\mathsf{j}}
\newcommand{\ssk}{\mathsf{k}}
\newcommand{\ssl}{\mathsf{l}}
\newcommand{\ssm}{\mathsf{m}}
\newcommand{\ssn}{\mathsf{n}}
\newcommand{\sso}{\mathsf{o}}
\newcommand{\ssp}{\mathsf{p}}
\newcommand{\ssq}{\mathsf{q}}
\newcommand{\ssr}{\mathsf{r}}
\newcommand{\sss}{\mathsf{s}}
\newcommand{\sst}{\mathsf{t}}
\newcommand{\ssu}{\mathsf{u}}
\newcommand{\ssv}{\mathsf{v}}
\newcommand{\ssw}{\mathsf{w}}
\newcommand{\ssx}{\mathsf{x}}
\newcommand{\ssy}{\mathsf{y}}
\newcommand{\ssz}{\mathsf{z}}

% upper case
\newcommand{\ssA}{\mathsf{A}}
\newcommand{\ssB}{\mathsf{B}}
\newcommand{\ssC}{\mathsf{C}}
\newcommand{\ssD}{\mathsf{D}}
\newcommand{\ssE}{\mathsf{E}}
\newcommand{\ssF}{\mathsf{F}}
\newcommand{\ssG}{\mathsf{G}}
\newcommand{\ssH}{\mathsf{H}}
\newcommand{\ssI}{\mathsf{I}}
\newcommand{\ssJ}{\mathsf{J}}
\newcommand{\ssK}{\mathsf{K}}
\newcommand{\ssL}{\mathsf{L}}
\newcommand{\ssM}{\mathsf{M}}
\newcommand{\ssN}{\mathsf{N}}
\newcommand{\ssO}{\mathsf{O}}
\newcommand{\ssP}{\mathsf{P}}
\newcommand{\ssQ}{\mathsf{Q}}
\newcommand{\ssR}{\mathsf{R}}
\newcommand{\ssS}{\mathsf{S}}
\newcommand{\ssT}{\mathsf{T}}
\newcommand{\ssU}{\mathsf{U}}
\newcommand{\ssV}{\mathsf{V}}
\newcommand{\ssW}{\mathsf{W}}
\newcommand{\ssX}{\mathsf{X}}
\newcommand{\ssY}{\mathsf{Y}}
\newcommand{\ssZ}{\mathsf{Z}}


%%%%% Boldface Math %%%%%%

% boldface sans serif
\safemath{\bmsa}{\bm{\ssa}}
\safemath{\bmsb}{\bm{\ssb}}
\safemath{\bmsc}{\bm{\ssc}}
\safemath{\bmsd}{\bm{\ssd}}
\safemath{\bmse}{\bm{\sse}}
\safemath{\bmsf}{\bm{\ssf}}
\safemath{\bmsg}{\bm{\ssg}}
\safemath{\bmsh}{\bm{\ssh}}
\safemath{\bmsi}{\bm{\ssi}}
\safemath{\bmsj}{\bm{\ssj}}
\safemath{\bmsk}{\bm{\ssk}}
\safemath{\bmsl}{\bm{\ssl}}
\safemath{\bmsm}{\bm{\ssm}}
\safemath{\bmsn}{\bm{\ssn}}
\safemath{\bmso}{\bm{\sso}}
\safemath{\bmsp}{\bm{\ssp}}
\safemath{\bmsq}{\bm{\ssq}}
\safemath{\bmsr}{\bm{\ssr}}
\safemath{\bmss}{\bm{\sss}}
\safemath{\bmst}{\bm{\sst}}
\safemath{\bmsu}{\bm{\ssu}}
\safemath{\bmsv}{\bm{\ssv}}
\safemath{\bmsw}{\bm{\ssw}}
\safemath{\bmsx}{\bm{\ssx}}
\safemath{\bmsy}{\bm{\ssy}}
\safemath{\bmsz}{\bm{\ssz}}

% boldface small upright math letters
\bmdefine{\bmualphad}{\upalpha}
\bmdefine{\bmubetad}{\upbeta}
\bmdefine{\bmuchid}{\upchi}
\bmdefine{\bmudeltad}{\updelta}
\bmdefine{\bmuepsilond}{\upepsilon}
\bmdefine{\bmuvarepsilond}{\upvarepsilon}
\bmdefine{\bmuetad}{\upeta}
\bmdefine{\bmugammad}{\upgamma}
\bmdefine{\bmuiotad}{\upiota}
\bmdefine{\bmukappad}{\upkappa}
\bmdefine{\bmulambdad}{\uplambda}
\bmdefine{\bmumud}{\upmu}
\bmdefine{\bmunud}{\upnu}
\bmdefine{\bmuomegad}{\upomega}
\bmdefine{\bmuphid}{\upphi}
\bmdefine{\bmuvarphid}{\upvarphi}
\bmdefine{\bmupid}{\uppi}
\bmdefine{\bmuvarpid}{\upvarpi}
\bmdefine{\bmupsid}{\uppsi}
\bmdefine{\bmurhod}{\uprho}
\bmdefine{\bmuvarrhod}{\upvarrho}
\bmdefine{\bmusigmad}{\upsigma}
\bmdefine{\bmuvarsigmad}{\upvarsigma}
\bmdefine{\bmutaud}{\uptau}
\bmdefine{\bmuthetad}{\uptheta}
\bmdefine{\bmuvarthetad}{\upvartheta}
\bmdefine{\bmuupsilond}{\upupsilon}
\bmdefine{\bmuxid}{\upxi}
\bmdefine{\bmuzetad}{\upzeta}

%---------------------------
\safemath{\bmua}{\mathbf{a}}
\safemath{\bmub}{\mathbf{b}}
\safemath{\bmuc}{\mathbf{c}}
\safemath{\bmud}{\mathbf{d}}
\safemath{\bmue}{\mathbf{e}}
\safemath{\bmuf}{\mathbf{f}}
\safemath{\bmug}{\mathbf{g}}
\safemath{\bmuh}{\mathbf{h}}
\safemath{\bmui}{\mathbf{i}}
\safemath{\bmuj}{\mathbf{j}}
\safemath{\bmuk}{\mathbf{k}}
\safemath{\bmul}{\mathbf{l}}
\safemath{\bmum}{\mathbf{m}}
\safemath{\bmun}{\mathbf{n}}
\safemath{\bmuo}{\mathbf{o}}
\safemath{\bmup}{\mathbf{p}}
\safemath{\bmuq}{\mathbf{q}}
\safemath{\bmur}{\mathbf{r}}
\safemath{\bmus}{\mathbf{s}}
\safemath{\bmut}{\mathbf{t}}
\safemath{\bmuu}{\mathbf{u}}
\safemath{\bmuv}{\mathbf{v}}
\safemath{\bmuw}{\mathbf{w}}
\safemath{\bmux}{\mathbf{x}}
\safemath{\bmuy}{\mathbf{y}}
\safemath{\bmuz}{\mathbf{z}}


\safemath{\bmualpha}{\bmualphad}
\safemath{\bmubeta}{\bmubetad}
\safemath{\bmuchi}{\bumchid}
\safemath{\bmudelta}{\bmudeltad}
\safemath{\bmuepsilon}{\bmuepsilond}
\safemath{\bmuvarepsilon}{\bmuvarepsilond}
\safemath{\bmueta}{\bmuetad}
\safemath{\bmugamma}{\bmugammad}
\safemath{\bmuiota}{\bmuiotad}
\safemath{\bmukappa}{\bmukappad}
\safemath{\bmulambda}{\bmulambdad}
\safemath{\bmumu}{\bmumud}
\safemath{\bmunu}{\bmunud}
\safemath{\bmuomega}{\bmuomegad}
\safemath{\bmuphi}{\bmuphid}
\safemath{\bmuvarphi}{\bmuvarphid}
\safemath{\bmupi}{\bmupid}
\safemath{\bmuvarpi}{\bmuvarpid}
\safemath{\bmupsi}{\bmupsid}
\safemath{\bmurho}{\bmurhod}
\safemath{\bmuvarrho}{\bmuvarrhod}
\safemath{\bmusigma}{\bmusigmad}
\safemath{\bmuvarsigma}{\bmuvarsigmad}
\safemath{\bmutau}{\bmutaud}
\safemath{\bmutheta}{\bmuthetad}
\safemath{\bmuvartheta}{\bmuvarthetad}
\safemath{\bmuupsilon}{\bmuupsilond}
\safemath{\bmuxi}{\bmuxid}
\safemath{\bmuzeta}{\bmuzetad}

% boldface small italic math letters
\bmdefine{\bmiad}{a}
\bmdefine{\bmibd}{b}
\bmdefine{\bmicd}{c}
\bmdefine{\bmidd}{d}
\bmdefine{\bmied}{e}
\bmdefine{\bmifd}{f}
\bmdefine{\bmigd}{g}
\bmdefine{\bmihd}{h}
\bmdefine{\bmiid}{i}
\bmdefine{\bmijd}{j}
\bmdefine{\bmikd}{k}
\bmdefine{\bmild}{l}
\bmdefine{\bmimd}{m}
\bmdefine{\bmind}{n}
\bmdefine{\bmiod}{o}
\bmdefine{\bmipd}{p}
\bmdefine{\bmiqd}{q}
\bmdefine{\bmird}{r}
\bmdefine{\bmisd}{s}
\bmdefine{\bmitd}{t}
\bmdefine{\bmiud}{u}
\bmdefine{\bmivd}{v}
\bmdefine{\bmiwd}{w}
\bmdefine{\bmixd}{x}
\bmdefine{\bmiyd}{y}
\bmdefine{\bmizd}{z}

\bmdefine{\bmialphad}{\alpha}
\bmdefine{\bmibetad}{\beta}
\bmdefine{\bmichid}{\chi}
\bmdefine{\bmideltad}{\delta}
\bmdefine{\bmiepsilond}{\epsilon}
\bmdefine{\bmivarepsilond}{\varepsilon}
\bmdefine{\bmietad}{\eta}
\bmdefine{\bmigammad}{\gamma}
\bmdefine{\bmiiotad}{\iota}
\bmdefine{\bmikappad}{\kappa}
\bmdefine{\bmivarkappad}{\varkappa}
\bmdefine{\bmilambdad}{\lambda}
\bmdefine{\bmimud}{\mu}
\bmdefine{\bminud}{\nu}
\bmdefine{\bmiomegad}{\omega}
\bmdefine{\bmiphid}{\phi}
\bmdefine{\bmivarphid}{\varphi}
\bmdefine{\bmipid}{\pi}
\bmdefine{\bmivarpid}{\varpi}
\bmdefine{\bmipsid}{\psi}
\bmdefine{\bmirhod}{\rho}
\bmdefine{\bmivarrhod}{\varrho}
\bmdefine{\bmisigmad}{\sigma}
\bmdefine{\bmivarsigmad}{\varsigma}
\bmdefine{\bmitaud}{\tau}
\bmdefine{\bmithetad}{\theta}
\bmdefine{\bmivarthetad}{\vartheta}
\bmdefine{\bmiupsilond}{\upsilon}
\bmdefine{\bmixid}{\xi}
\bmdefine{\bmizetad}{\zeta}

%----------------------
\safemath{\bmia}{\bmiad}
\safemath{\bmib}{\bmibd}
\safemath{\bmic}{\bmicd}
\safemath{\bmid}{\bmidd}
\safemath{\bmie}{\bmied}
\safemath{\bmif}{\bmifd}
\safemath{\bmig}{\bmigd}
\safemath{\bmih}{\bmihd}
\safemath{\bmii}{\bmiid}
\safemath{\bmij}{\bmijd}
\safemath{\bmik}{\bmikd}
\safemath{\bmil}{\bmild}
\safemath{\bmim}{\bmimd}
\safemath{\bmin}{\bmind}
\safemath{\bmio}{\bmiod}
\safemath{\bmip}{\bmipd}
\safemath{\bmiq}{\bmiqd}
\safemath{\bmir}{\bmird}
\safemath{\bmis}{\bmisd}
\safemath{\bmit}{\bmitd}
\safemath{\bmiu}{\bmiud}
\safemath{\bmiv}{\bmivd}
\safemath{\bmiw}{\bmiwd}
\safemath{\bmix}{\bmixd}
\safemath{\bmiy}{\bmiyd}
\safemath{\bmiz}{\bmizd}

\safemath{\bmialpha}{\bmialphad}
\safemath{\bmibeta}{\bmibetad}
\safemath{\bmichi}{\bmichid}
\safemath{\bmidelta}{\bmideltad}
\safemath{\bmiepsilon}{\bmiepsilond}
\safemath{\bmivarepsilon}{\bmivarepsilond}
\safemath{\bmieta}{\bmietad}
\safemath{\bmigamma}{\bmigammad}
\safemath{\bmiiota}{\bmiiotad}
\safemath{\bmikappa}{\bmikappad}
\safemath{\bmivarkappa}{\bmivarkappad}
\safemath{\bmilambda}{\bmilambdad}
\safemath{\bmimu}{\bmimud}
\safemath{\bminu}{\bminud}
\safemath{\bmiomega}{\bmiomegad}
\safemath{\bmiphi}{\bmiphid}
\safemath{\bmivarphi}{\bmivarphid}
\safemath{\bmipi}{\bmipid}
\safemath{\bmivarpi}{\bmivarpid}
\safemath{\bmipsi}{\bmipsid}
\safemath{\bmirho}{\bmirhod}
\safemath{\bmivarrho}{\bmivarrhod}
\safemath{\bmisigma}{\bmisigmad}
\safemath{\bmivarsigma}{\bmivarsigmad}
\safemath{\bmitau}{\bmitaud}
\safemath{\bmitheta}{\bmithetad}
\safemath{\bmivartheta}{\bmivarthetad}
\safemath{\bmiupsilon}{\bmiupsilond}
\safemath{\bmixi}{\bmixid}
\safemath{\bmizeta}{\bmizetad}


% boldface capital upright math letters
\bmdefine{\bmuDeltad}{\Updelta}
\bmdefine{\bmuGammad}{\Upgamma}
\bmdefine{\bmuLambdad}{\Uplambda}
\bmdefine{\bmuOmegad}{\Upomega}
\bmdefine{\bmuPhid}{\Upphi}
\bmdefine{\bmuPid}{\Uppi}
\bmdefine{\bmuPsid}{\Uppsi}
\bmdefine{\bmuSigmad}{\Upsigma}
\bmdefine{\bmuThetad}{\Uptheta}
\bmdefine{\bmuUpsilond}{\Upupsilon}
\bmdefine{\bmuXid}{\Upxi}

%---------------------------
\safemath{\bmuA}{\mathbf{A}}
\safemath{\bmuB}{\mathbf{B}}
\safemath{\bmuC}{\mathbf{C}}
\safemath{\bmuD}{\mathbf{D}}
\safemath{\bmuE}{\mathbf{E}}
\safemath{\bmuF}{\mathbf{F}}
\safemath{\bmuG}{\mathbf{G}}
\safemath{\bmuH}{\mathbf{H}}
\safemath{\bmuI}{\mathbf{I}}
\safemath{\bmuJ}{\mathbf{J}}
\safemath{\bmuK}{\mathbf{K}}
\safemath{\bmuL}{\mathbf{L}}
\safemath{\bmuM}{\mathbf{M}}
\safemath{\bmuN}{\mathbf{N}}
\safemath{\bmuO}{\mathbf{O}}
\safemath{\bmuP}{\mathbf{P}}
\safemath{\bmuQ}{\mathbf{Q}}
\safemath{\bmuR}{\mathbf{R}}
\safemath{\bmuS}{\mathbf{S}}
\safemath{\bmuT}{\mathbf{T}}
\safemath{\bmuU}{\mathbf{U}}
\safemath{\bmuV}{\mathbf{V}}
\safemath{\bmuW}{\mathbf{W}}
\safemath{\bmuX}{\mathbf{X}}
\safemath{\bmuY}{\mathbf{Y}}
\safemath{\bmuZ}{\mathbf{Z}}

\safemath{\bmuZero}{\mathbf{0}}
\safemath{\bmuOne}{\mathbf{1}}

\safemath{\bmuDelta}{\bmuDeltad}
\safemath{\bmuGamma}{\bmuGammad}
\safemath{\bmuLambda}{\bmuLambdad}
\safemath{\bmuOmega}{\bmuOmegad}
\safemath{\bmuPhi}{\bmuPhid}
\safemath{\bmuPi}{\bmuPid}
\safemath{\bmuPsi}{\bmuPsid}
\safemath{\bmuSigma}{\bmuSigmad}
\safemath{\bmuTheta}{\bmuThetad}
\safemath{\bmuUpsilon}{\bmuUpsilond}
\safemath{\bmuXi}{\bmuXid}



% boldface capital italic math letters
\bmdefine{\bmiAd}{A}
\bmdefine{\bmiBd}{B}
\bmdefine{\bmiCd}{C}
\bmdefine{\bmiDd}{D}
\bmdefine{\bmiEd}{E}
\bmdefine{\bmiFd}{F}
\bmdefine{\bmiGd}{G}
\bmdefine{\bmiHd}{H}
\bmdefine{\bmiId}{I}
\bmdefine{\bmiJd}{J}
\bmdefine{\bmiKd}{K}
\bmdefine{\bmiLd}{L}
\bmdefine{\bmiMd}{M}
\bmdefine{\bmiOd}{N}
\bmdefine{\bmiPd}{O}
\bmdefine{\bmiQd}{P}
\bmdefine{\bmiRd}{R}
\bmdefine{\bmiSd}{S}
\bmdefine{\bmiTd}{T}
\bmdefine{\bmiUd}{U}
\bmdefine{\bmiVd}{V}
\bmdefine{\bmiWd}{W}
\bmdefine{\bmiXd}{X}
\bmdefine{\bmiYd}{Y}
\bmdefine{\bmiZd}{Z}

\bmdefine{\bmiDeltad}{\Delta}
\bmdefine{\bmiGammad}{\Gamma}
\bmdefine{\bmiLambdad}{\Lambda}
\bmdefine{\bmiOmegad}{\Omega}
\bmdefine{\bmiPhid}{\Phi}
\bmdefine{\bmiPid}{\Pi}
\bmdefine{\bmiPsid}{\Psi}
\bmdefine{\bmiSigmad}{\Sigma}
\bmdefine{\bmiThetad}{\Theta}
\bmdefine{\bmiUpsilond}{\Upsilon}
\bmdefine{\bmiXid}{\Xi}

%-----------------------
\safemath{\bmiA}{\bmiAd}
\safemath{\bmiB}{\bmiBd}
\safemath{\bmiC}{\bmiCd}
\safemath{\bmiD}{\bmiDd}
\safemath{\bmiE}{\bmiEd}
\safemath{\bmiF}{\bmiFd}
\safemath{\bmiG}{\bmiGd}
\safemath{\bmiH}{\bmiHd}
\safemath{\bmiI}{\bmiId}
\safemath{\bmiJ}{\bmiJd}
\safemath{\bmiK}{\bmiKd}
\safemath{\bmiL}{\bmiLd}
\safemath{\bmiM}{\bmiMd}
\safemath{\bmiN}{\bmiNd}
\safemath{\bmiO}{\bmiOd}
\safemath{\bmiP}{\bmiPd}
\safemath{\bmiQ}{\bmiQd}
\safemath{\bmiR}{\bmiRd}
\safemath{\bmiS}{\bmiSd}
\safemath{\bmiT}{\bmiTd}
\safemath{\bmiU}{\bmiUd}
\safemath{\bmiV}{\bmiVd}
\safemath{\bmiW}{\bmiWd}
\safemath{\bmiX}{\bmiXd}
\safemath{\bmiY}{\bmiYd}
\safemath{\bmiZ}{\bmiZd}

\safemath{\bmiDelta}{\bmiDeltad}
\safemath{\bmiGamma}{\bmiGammad}
\safemath{\bmiLambda}{\bmiLambdad}
\safemath{\bmiOmega}{\bmiOmegad}
\safemath{\bmiPhi}{\bmiPhid}
\safemath{\bmiPi}{\bmiPid}
\safemath{\bmiPsi}{\bmiPsid}
\safemath{\bmiSigma}{\bmiSigmad}
\safemath{\bmiTheta}{\bmiThetad}
\safemath{\bmiUpsilon}{\bmiUpsilond}
\safemath{\bmiXi}{\bmiXid}

%***********************************************************************


%%%%% Events %%%%%%%%%%%%%%%%%%
\safemath{\evA}{\mathcal{A}}
\safemath{\evB}{\mathcal{B}}
\safemath{\evC}{\mathcal{C}}
\safemath{\evD}{\mathcal{D}}
\safemath{\evE}{\mathcal{E}}
\safemath{\evF}{\mathcal{F}}
\safemath{\evG}{\mathcal{G}}
\safemath{\evH}{\mathcal{H}}
\safemath{\evI}{\mathcal{I}}
\safemath{\evJ}{\mathcal{J}}
\safemath{\evK}{\mathcal{K}}
\safemath{\evL}{\mathcal{L}}
\safemath{\evM}{\mathcal{M}}
\safemath{\evN}{\mathcal{N}}
\safemath{\evO}{\mathcal{O}}
\safemath{\evP}{\mathcal{P}}
\safemath{\evQ}{\mathcal{Q}}
\safemath{\evR}{\mathcal{R}}
\safemath{\evS}{\mathcal{S}}
\safemath{\evT}{\mathcal{T}}
\safemath{\evU}{\mathcal{U}}
\safemath{\evV}{\mathcal{V}}
\safemath{\evW}{\mathcal{W}}
\safemath{\evX}{\mathcal{X}}
\safemath{\evY}{\mathcal{Y}}
\safemath{\evZ}{\mathcal{Z}}


%%%%% Sets %%%%%%%%%%%%%%%%%%
\safemath{\setA}{\mathcal{A}}
\safemath{\setB}{\mathcal{B}}
\safemath{\setC}{\mathcal{C}}
\safemath{\setD}{\mathcal{D}}
\safemath{\setE}{\mathcal{E}}
\safemath{\setF}{\mathcal{F}}
\safemath{\setG}{\mathcal{G}}
\safemath{\setH}{\mathcal{H}}
\safemath{\setI}{\mathcal{I}}
\safemath{\setJ}{\mathcal{J}}
\safemath{\setK}{\mathcal{K}}
\safemath{\setL}{\mathcal{L}}
\safemath{\setM}{\mathcal{M}}
\safemath{\setN}{\mathcal{N}}
\safemath{\setO}{\mathcal{O}}
\safemath{\setP}{\mathcal{P}}
\safemath{\setQ}{\mathcal{Q}}
\safemath{\setR}{\mathcal{R}}
\safemath{\setS}{\mathcal{S}}
\safemath{\setT}{\mathcal{T}}
\safemath{\setU}{\mathcal{U}}
\safemath{\setV}{\mathcal{V}}
\safemath{\setW}{\mathcal{W}}
\safemath{\setX}{\mathcal{X}}
\safemath{\setY}{\mathcal{Y}}
\safemath{\setZ}{\mathcal{Z}}
\safemath{\emptySet}{\varnothing}

%%%%% Collections %%%%%%%%%%%%%%%%%%
\safemath{\colA}{\mathscr{A}}
\safemath{\colB}{\mathscr{B}}
\safemath{\colC}{\mathscr{C}}
\safemath{\colD}{\mathscr{D}}
\safemath{\colE}{\mathscr{E}}
\safemath{\colF}{\mathscr{F}}
\safemath{\colG}{\mathscr{G}}
\safemath{\colH}{\mathscr{H}}
\safemath{\colI}{\mathscr{I}}
\safemath{\colJ}{\mathscr{J}}
\safemath{\colK}{\mathscr{K}}
\safemath{\colL}{\mathscr{L}}
\safemath{\colM}{\mathscr{M}}
\safemath{\colN}{\mathscr{N}}
\safemath{\colO}{\mathscr{O}}
\safemath{\colP}{\mathscr{P}}
\safemath{\colQ}{\mathscr{Q}}
\safemath{\colR}{\mathscr{R}}
\safemath{\colS}{\mathscr{S}}
\safemath{\colT}{\mathscr{T}}
\safemath{\colU}{\mathscr{U}}
\safemath{\colV}{\mathscr{V}}
\safemath{\colW}{\mathscr{W}}
\safemath{\colX}{\mathscr{X}}
\safemath{\colY}{\mathscr{Y}}
\safemath{\colZ}{\mathscr{Z}}


%%%%% Operators %%%%%%%%%%%
\safemath{\opA}{\mathbb{A}}
\safemath{\opB}{\mathbb{B}}
\safemath{\opC}{\mathbb{C}}
\safemath{\opD}{\mathbb{D}}
\safemath{\opE}{\mathbb{E}}
\safemath{\opF}{\mathbb{F}}
\safemath{\opG}{\mathbb{G}}
\safemath{\opH}{\mathbb{H}}
\safemath{\opI}{\mathbb{I}}
\safemath{\opJ}{\mathbb{J}}
\safemath{\opK}{\mathbb{K}}
\safemath{\opL}{\mathbb{L}}
\safemath{\opM}{\mathbb{M}}
\safemath{\opN}{\mathbb{N}}
\safemath{\opO}{\mathbb{O}}
\safemath{\opP}{\mathbb{P}}
\safemath{\opQ}{\mathbb{Q}}
\safemath{\opR}{\mathbb{R}}
\safemath{\opS}{\mathbb{S}}
\safemath{\opT}{\mathbb{T}}
\safemath{\opU}{\mathbb{U}}
\safemath{\opV}{\mathbb{V}}
\safemath{\opW}{\mathbb{W}}
\safemath{\opX}{\mathbb{X}}
\safemath{\opY}{\mathbb{Y}}
\safemath{\opZ}{\mathbb{Z}}
\safemath{\opZero}{\mathbb{O}}
\safemath{\identityop}{\opI}


%%%%%%%%%%%% Scalars %%%%%%%%%%%%%%%%%%%

\safemath{\sca}{a}
\safemath{\scb}{b}
\safemath{\scc}{c}
\safemath{\scd}{d}
\safemath{\sce}{e}
\safemath{\scf}{f}
\safemath{\scg}{g}
\safemath{\sch}{h}
\safemath{\sci}{i}
\safemath{\scj}{j}
\safemath{\sck}{k}
\safemath{\scl}{l}
\safemath{\scm}{m}
\safemath{\scn}{n}
\safemath{\sco}{o}
\safemath{\scp}{p}
\safemath{\scq}{q}
\safemath{\scr}{r}
\safemath{\scs}{s}
\safemath{\sct}{t}
\safemath{\scu}{u}
\safemath{\scv}{v}
\safemath{\scw}{w}
\safemath{\scx}{x}
\safemath{\scy}{y}
\safemath{\scz}{z}

\safemath{\scA}{A}
\safemath{\scB}{B}
\safemath{\scC}{C}
\safemath{\scD}{D}
\safemath{\scE}{E}
\safemath{\scF}{F}
\safemath{\scG}{G}
\safemath{\scH}{H}
\safemath{\scI}{I}
\safemath{\scJ}{J}
\safemath{\scK}{K}
\safemath{\scL}{L}
\safemath{\scM}{M}
\safemath{\scN}{N}
\safemath{\scO}{O}
\safemath{\scP}{P}
\safemath{\scQ}{Q}
\safemath{\scR}{R}
\safemath{\scS}{S}
\safemath{\scT}{T}
\safemath{\scU}{U}
\safemath{\scV}{V}
\safemath{\scW}{W}
\safemath{\scX}{X}
\safemath{\scY}{Y}
\safemath{\scZ}{Z}

\safemath{\scalpha}{\alpha}
\safemath{\scbeta}{\beta}
\safemath{\scchi}{\chi}
\safemath{\scdelta}{\delta}
\safemath{\scepsilon}{\epsilon}
\safemath{\scvarepsilon}{\varepsilon}
\safemath{\sceta}{\eta}
\safemath{\scgamma}{\gamma}
\safemath{\sciota}{\iota}
\safemath{\sckappa}{\kappa}
\safemath{\scvarkappa}{\varkappa}
\safemath{\sclambda}{\lambda}
\safemath{\scmu}{\mu}
\safemath{\scnu}{\nu}
\safemath{\scomega}{\omega}
\safemath{\scphi}{\phi}
\safemath{\scvarphi}{\varphi}
\safemath{\scpi}{\pi}
\safemath{\scvarpi}{\varpi}
\safemath{\scpsi}{\psi}
\safemath{\scrho}{\rho}
\safemath{\scvarrho}{\varrho}
\safemath{\scsigma}{\sigma}
\safemath{\scvarsigma}{\varsigma}
\safemath{\sctau}{\tau}
\safemath{\sctheta}{\theta}
\safemath{\scvartheta}{\vartheta}
\safemath{\scupsilon}{\upsilon}
\safemath{\scxi}{\xi}
\safemath{\sczeta}{\zeta}


%%%%%%%%%%%% Vectors %%%%%%%%%%%%%%%

\safemath{\veca}{\mathbf{a}}
\safemath{\vecb}{\mathbf{b}}
\safemath{\vecc}{\mathbf{c}}
\safemath{\vecd}{\mathbf{d}}
\safemath{\vece}{\mathbf{e}}
\safemath{\vecf}{\mathbf{f}}
\safemath{\vecg}{\mathbf{g}}
\safemath{\vech}{\mathbf{h}}
\safemath{\veci}{\mathbf{i}}
\safemath{\vecj}{\mathbf{j}}
\safemath{\veck}{\mathbf{k}}
\safemath{\vecl}{\mathbf{l}}
\safemath{\vecm}{\mathbf{m}}
\safemath{\vecn}{\mathbf{n}}
\safemath{\veco}{\mathbf{o}}
\safemath{\vecp}{\mathbf{p}}
\safemath{\vecq}{\mathbf{q}}
\safemath{\vecr}{\mathbf{r}}
\safemath{\vecs}{\mathbf{s}}
\safemath{\vect}{\mathbf{t}}
\safemath{\vecu}{\mathbf{u}}
\safemath{\vecv}{\mathbf{v}}
\safemath{\vecw}{\mathbf{w}}
\safemath{\vecx}{\mathbf{x}}
\safemath{\vecy}{\mathbf{y}}
\safemath{\vecz}{\mathbf{z}}
\safemath{\veczero}{\mathbf{0}}
\safemath{\vecone}{\mathbf{1}}

\safemath{\vecalpha}{\upalpha}
\safemath{\vecbeta}{\upbeta}
\safemath{\vecchi}{\upchi}
\safemath{\vecdelta}{\updelta}
\safemath{\vecepsilon}{\upepsilon}
\safemath{\vecvarepsilon}{\upvarepsilon}
\safemath{\veceta}{\upeta}
\safemath{\vecgamma}{\upgamma}
\safemath{\veciota}{\upiota}
\safemath{\veckappa}{\upkappa}
\safemath{\veclambda}{\uplambda}
\safemath{\vecmu}{\text{\textmu}}
\safemath{\vecnu}{\upnu}
\safemath{\vecomega}{\upomega}
\safemath{\vecphi}{\upphi}
\safemath{\vecvarphi}{\upvarphi}
\safemath{\vecpi}{\uppi}
\safemath{\vecvarpi}{\upvarpi}
\safemath{\vecpsi}{\uppsi}
\safemath{\vecrho}{\uprho}
\safemath{\vecvarrho}{\upvarrho}
\safemath{\vecsigma}{\upsigma}
\safemath{\vecvarsigma}{\upvarsigma}
\safemath{\vectau}{\uptau}
\safemath{\vectheta}{\uptheta}
\safemath{\vecvartheta}{\upvartheta}
\safemath{\vecupsilon}{\upupsilon}
\safemath{\vecxi}{\upxi}
\safemath{\veczeta}{\upzeta}

%%%%%%%%%%%% Vector components %%%%%%%%%%%%%%%

\safemath{\vecac}{a}
\safemath{\vecbc}{b}
\safemath{\veccc}{c}
\safemath{\vecdc}{d}
\safemath{\vecec}{e}
\safemath{\vecfc}{f}
\safemath{\vecgc}{g}
\safemath{\vechc}{h}
\safemath{\vecic}{i}
\safemath{\vecjc}{j}
\safemath{\veckc}{k}
\safemath{\veclc}{l}
\safemath{\vecmc}{m}
\safemath{\vecnc}{n}
\safemath{\vecoc}{o}
\safemath{\vecpc}{p}
\safemath{\vecqc}{q}
\safemath{\vecrc}{r}
\safemath{\vecsc}{s}
\safemath{\vectc}{t}
\safemath{\vecuc}{u}
\safemath{\vecvc}{v}
\safemath{\vecwc}{w}
\safemath{\vecxc}{x}
\safemath{\vecyc}{y}
\safemath{\veczc}{z}


%%%%%%%%%%%%%%% Matrices %%%%%%%%%%%%%%%

\safemath{\matA}{\mathbf{A}}
\safemath{\matB}{\mathbf{B}}
\safemath{\matC}{\mathbf{C}}
\safemath{\matD}{\mathbf{D}}
\safemath{\matE}{\mathbf{E}}
\safemath{\matF}{\mathbf{F}}
\safemath{\matG}{\mathbf{G}}
\safemath{\matH}{\mathbf{H}}
\safemath{\matI}{\mathbf{I}}
\safemath{\matJ}{\mathbf{J}}
\safemath{\matK}{\mathbf{K}}
\safemath{\matL}{\mathbf{L}}
\safemath{\matM}{\mathbf{M}}
\safemath{\matN}{\mathbf{N}}
\safemath{\matO}{\mathbf{O}}
\safemath{\matP}{\mathbf{P}}
\safemath{\matQ}{\mathbf{Q}}
\safemath{\matR}{\mathbf{R}}
\safemath{\matS}{\mathbf{S}}
\safemath{\matT}{\mathbf{T}}
\safemath{\matU}{\mathbf{U}}
\safemath{\matV}{\mathbf{V}}
\safemath{\matW}{\mathbf{W}}
\safemath{\matX}{\mathbf{X}}
\safemath{\matY}{\mathbf{Y}}
\safemath{\matZ}{\mathbf{Z}}
\safemath{\matzero}{\mathbf{0}}

\safemath{\matDelta}{\Updelta}
\safemath{\matGamma}{\Upgammma}
\safemath{\matLambda}{\Uplambda}
\safemath{\matOmega}{\Upomega}
\safemath{\matPhi}{\Upphi}
\safemath{\matPi}{\Uppi}
\safemath{\matPsi}{\Uppsi}
\safemath{\matSigma}{\Upsigma}
\safemath{\matTheta}{\Uptheta}
\safemath{\matUpsilon}{\Upupsilon}
\safemath{\matXi}{\Upxi}

\safemath{\matidentity}{\matI}
\safemath{\matone}{\matO}


%%%%%% Matrix components %%%%%%
\safemath{\matAc}{a}
\safemath{\matBc}{b}
\safemath{\matCc}{c}
\safemath{\matDc}{d}
\safemath{\matEc}{e}
\safemath{\matFc}{f}
\safemath{\matGc}{g}
\safemath{\matHc}{h}
\safemath{\matIc}{i}
\safemath{\matJc}{j}
\safemath{\matKc}{k}
\safemath{\matLc}{l}
\safemath{\matMc}{m}
\safemath{\matNc}{n}
\safemath{\matOc}{o}
\safemath{\matPc}{p}
\safemath{\matQc}{q}
\safemath{\matRc}{r}
\safemath{\matSc}{s}
\safemath{\matTc}{t}
\safemath{\matUc}{u}
\safemath{\matVc}{v}
\safemath{\matWc}{w}
\safemath{\matXc}{x}
\safemath{\matYc}{y}
\safemath{\matZc}{z}


%%%%%% Random scalars, vectors and matrices %%%%%%%%

% random scalars
\safemath{\rnda}{\bmia}
\safemath{\rndb}{\bmib}
\safemath{\rndc}{\bmic}
\safemath{\rndd}{\bmid}
\safemath{\rnde}{\bmie}
\safemath{\rndf}{\bmif}
\safemath{\rndg}{\bmig}
\safemath{\rndh}{\bmih}
\safemath{\rndi}{\bmii}
\safemath{\rndj}{\bmij}
\safemath{\rndk}{\bmik}
\safemath{\rndl}{\bmil}
\safemath{\rndm}{\bmim}
\safemath{\rndn}{\bmin}
\safemath{\rndo}{\bmio}
\safemath{\rndp}{\bmip}
\safemath{\rndq}{\bmiq}
\safemath{\rndr}{\bmir}
\safemath{\rnds}{\bmis}
\safemath{\rndt}{\bmit}
\safemath{\rndu}{\bmiu}
\safemath{\rndv}{\bmiv}
\safemath{\rndw}{\bmiw}
\safemath{\rndx}{\bmix}
\safemath{\rndy}{\bmiy}
\safemath{\rndz}{\bmiz}

\safemath{\rndA}{\bmiA}
\safemath{\rndB}{\bmiB}
\safemath{\rndC}{\bmiC}
\safemath{\rndD}{\bmiD}
\safemath{\rndE}{\bmiE}
\safemath{\rndF}{\bmiF}
\safemath{\rndG}{\bmiG}
\safemath{\rndH}{\bmiH}
\safemath{\rndI}{\bmiI}
\safemath{\rndJ}{\bmiJ}
\safemath{\rndK}{\bmiK}
\safemath{\rndL}{\bmiL}
\safemath{\rndM}{\bmiM}
\safemath{\rndN}{\bmiN}
\safemath{\rndO}{\bmiO}
\safemath{\rndP}{\bmiP}
\safemath{\rndQ}{\bmiQ}
\safemath{\rndR}{\bmiR}
\safemath{\rndS}{\bmiS}
\safemath{\rndT}{\bmiT}
\safemath{\rndU}{\bmiU}
\safemath{\rndV}{\bmiV}
\safemath{\rndW}{\bmiW}
\safemath{\rndX}{\bmiX}
\safemath{\rndY}{\bmiY}
\safemath{\rndZ}{\bmiZ}

\safemath{\rndalpha}{\bmialpha}
\safemath{\rndbeta}{\bmibeta}
\safemath{\rndchi}{\bmichi}
\safemath{\rnddelta}{\bmidelta}
\safemath{\rndepsilon}{\bmiepsilon}
\safemath{\rndvarepsilon}{\bmivarepsilon}
\safemath{\rndeta}{\bmieta}
\safemath{\rndgamma}{\bmigamma}
\safemath{\rndiota}{\bmiiota}
\safemath{\rndkappa}{\bmikappa}
\safemath{\rndlambda}{\bmilambda}
\safemath{\rndmu}{\bmimu}
\safemath{\rndnu}{\bminu}
\safemath{\rndomega}{\bmiomega}
\safemath{\rndphi}{\bmiphi}
\safemath{\rndvarphi}{\bmivarphi}
\safemath{\rndpi}{\bmipi}
\safemath{\rndvarpi}{\bmivarpi}
\safemath{\rndpsi}{\bmipsi}
\safemath{\rndrho}{\bmirho}
\safemath{\rndvarrho}{\bmivarrho}
\safemath{\rndsigma}{\bmisigma}
\safemath{\rndvarsigma}{\bmivarsigma}
\safemath{\rndtau}{\bmitau}
\safemath{\rndtheta}{\bmitheta}
\safemath{\rndvartheta}{\bmivartheta}
\safemath{\rndupsilon}{\bmiupsilon}
\safemath{\rndxi}{\bmixi}
\safemath{\rndzeta}{\bmizeta}

% random vectors
\safemath{\rveca}{\bmua}
\safemath{\rvecb}{\bmub}
\safemath{\rvecc}{\bmuc}
\safemath{\rvecd}{\bmud}
\safemath{\rvece}{\bmue}
\safemath{\rvecf}{\bmuf}
\safemath{\rvecg}{\bmug}
\safemath{\rvech}{\bmuh}
\safemath{\rveci}{\bmui}
\safemath{\rvecj}{\bmuj}
\safemath{\rveck}{\bmuk}
\safemath{\rvecl}{\bmul}
\safemath{\rvecm}{\bmum}
\safemath{\rvecn}{\bmun}
\safemath{\rveco}{\bmuo}
\safemath{\rvecp}{\bmup}
\safemath{\rvecq}{\bmuq}
\safemath{\rvecr}{\bmur}
\safemath{\rvecs}{\bmus}
\safemath{\rvect}{\bmut}
\safemath{\rvecu}{\bmuu}
\safemath{\rvecv}{\bmuv}
\safemath{\rvecw}{\bmuw}
\safemath{\rvecx}{\bmux}
\safemath{\rvecy}{\bmuy}
\safemath{\rvecz}{\bmuz}

\safemath{\rvecalpha}{\bmualpha}
\safemath{\rvecbeta}{\bmubeta}
\safemath{\rvecchi}{\bmuchi}
\safemath{\rvecdelta}{\bmudelta}
\safemath{\rvecepsilon}{\bmuepsilon}
\safemath{\rvecvarepsilon}{\bmuvarepsilon}
\safemath{\rveceta}{\bmueta}
\safemath{\rvecgamma}{\bmugamma}
\safemath{\rveciota}{\bmuiota}
\safemath{\rveckappa}{\bmukappa}
\safemath{\rveclambda}{\bmulambda}
\safemath{\rvecmu}{\bmumu}
\safemath{\rvecnu}{\bmunu}
\safemath{\rvecomega}{\bmuomega}
\safemath{\rvecphi}{\bmuphi}
\safemath{\rvecvarphi}{\bmuvarphi}
\safemath{\rvecpi}{\bmupi}
\safemath{\rvecvarpi}{\bmuvarpi}
\safemath{\rvecpsi}{\bmupsi}
\safemath{\rvecrho}{\bmurho}
\safemath{\rvecvarrho}{\bmuvarrho}
\safemath{\rvecsigma}{\bmusigma}
\safemath{\rvecvarsigma}{\bmuvarsigma}
\safemath{\rvectau}{\bmutau}
\safemath{\rvectheta}{\bmutheta}
\safemath{\rvecvartheta}{\bmuvartheta}
\safemath{\rvecupsilon}{\bmuupsilon}
\safemath{\rvecxi}{\bmuxi}
\safemath{\rveczeta}{\bmuzeta}


% random matrices
\safemath{\rmatA}{\bmuA}
\safemath{\rmatB}{\bmuB}
\safemath{\rmatC}{\bmuC}
\safemath{\rmatD}{\bmuD}
\safemath{\rmatE}{\bmuE}
\safemath{\rmatF}{\bmuF}
\safemath{\rmatG}{\bmuG}
\safemath{\rmatH}{\bmuH}
\safemath{\rmatI}{\bmuI}
\safemath{\rmatJ}{\bmuJ}
\safemath{\rmatK}{\bmuK}
\safemath{\rmatL}{\bmuL}
\safemath{\rmatM}{\bmuM}
\safemath{\rmatN}{\bmuN}
\safemath{\rmatO}{\bmuO}
\safemath{\rmatP}{\bmuP}
\safemath{\rmatQ}{\bmuQ}
\safemath{\rmatR}{\bmuR}
\safemath{\rmatS}{\bmuS}
\safemath{\rmatT}{\bmuT}
\safemath{\rmatU}{\bmuU}
\safemath{\rmatV}{\bmuV}
\safemath{\rmatW}{\bmuW}
\safemath{\rmatX}{\bmuX}
\safemath{\rmatY}{\bmuY}
\safemath{\rmatZ}{\bmuZ}

\safemath{\rmatDelta}{\bmuDelta}
\safemath{\rmatGamma}{\bmuGamma}
\safemath{\rmatLambda}{\bmuLambda}
\safemath{\rmatOmega}{\bmuOmega}
\safemath{\rmatPhi}{\bmuPhi}
\safemath{\rmatPi}{\bmuPi}
\safemath{\rmatPsi}{\bmuPsi}
\safemath{\rmatSigma}{\bmuSigma}
\safemath{\rmatTheta}{\bmuTheta}
\safemath{\rmatUpsilon}{\bmuUpsilon}
\safemath{\rmatXi}{\bmuXi}


%%%%% New environments %%%%%%%

% tighter spacing for a inline matrix 
\newenvironment{textbmatrix}{	\setlength{\arraycolsep}{2.5pt}%
								\big[\begin{matrix}}{\end{matrix}\big]%
								\raisebox{0.08ex}{\vphantom{M}}}
								

%%%%% Short forms for environments %%%%%

% \def\be{\begin{equation}}
% \def\ee{\end{equation}}
% \def\een{\nonumber \end{equation}}
% \def\mat{\begin{bmatrix}}
% \def\emat{\end{bmatrix}}
 \def\btm{\begin{textbmatrix}}
 \def\etm{\end{textbmatrix}}

% \def\ba#1\ea{\begin{align}#1\end{align}}
% \def\bas#1\eas{\begin{align*}#1\end{align*}}
% \def\bs#1\es{\begin{split}#1\end{split}} 
% \def\bg#1\eg{\begin{gather}#1\end{gather}}
% \def\bml#1\eml{\begin{multline}#1\end{multline}}
% \def\bi#1\ei{\begin{itemize}#1\end{itemize}} 
% \def\bipi#1\eipi{\begin{inparaitem}#1\end{inparaitem}}

%%%%% Useful abbreviations %%%%%

%\newcommand{\safemath}[2]{\newcommand{#1}{\ensuremath{#2}\xspace}}
% now in vmr-symbols-*.tex
\newcommand{\subtext}[1]{\text{\fontfamily{cmr}\fontshape{n}\fontseries{m}\selectfont{}#1}}
\newcommand{\lefto}{\mathopen{}\left}
\newcommand{\Disp}{\displaystyle}
\newcommand{\sub}[1]{\ensuremath{_{\subtext{#1}}}} % for text mode subscripts

%%%%% for operator alignment in broken equations in the AMS align environment
\newcommand{\dummyrel}[1]{\mathrel{\hphantom{#1}}\strut\mskip-\medmuskip}

%%%%% Operators %%%%%

%\DeclareMathOperator{\tr}{tr}				% trace
%\DeclareMathOperator{\Tr}{\opT r}			% Trace
%\DeclareMathOperator{\diag}{diag}			% diagonal matrix
%\DeclareMathOperator{\dg}{\opD}				% diagonal matrix
%\DeclareMathOperator{\rank}{rank}			% rank of a matrix
\DeclareMathOperator{\spark}{spark}			% spark of a matrix
%\DeclareMathOperator{\ker}{ker}			% kernel of a matrix
%\DeclareMathOperator{\adj}{adj}				% adjunct matrix
\DeclareMathOperator{\vt}{\opV}				% vectorization
\newcommand{\vectorize}[1]{\ensuremath{\mathbb{V}\text{ec}(#1)}} % Vec(X)
\DeclareMathOperator{\rect}{rect}			% rect function
\DeclareMathOperator{\sign}{sign}			% signum
\DeclareMathOperator{\sinc}{sinc}			% sinc function
\DeclareMathOperator{\elem}{\in}				% element of
%\DeclareMathOperator{\dom}{dom}				% domain of a function
%\DeclareMathOperator{\rng}{rng}				% range of a function
\DeclareMathOperator{\interior}{int}			% interior of a set
\DeclareMathOperator*{\argmin}{arg\;min}		% arg min
\DeclareMathOperator*{\argmax}{arg\;max}		% arg max
\DeclareMathOperator*{\limm}{l.i.m.\,}		% limit in the mean
\DeclareMathOperator{\kron}{\otimes}			% Kroneker Product
\DeclareMathOperator{\had}{\odot}			% Hadamard Product
\DeclareMathOperator{\four}{\opF}			% Fourier transform
\DeclareMathOperator{\Exop}{\opE}			% expectation operator
\DeclareMathOperator{\Varop}{\opV\!\mathrm{ar}} % variance operator
\DeclareMathOperator{\Covop}{\opC\!\mathrm{ov}}% covariance operator
\DeclareMathOperator{\conv}{\star}			% convolution operator
\DeclareMathOperator{\spn}{span}			 	% span of a set of vectors
\DeclareMathOperator{\cspn}{\clos{\spn}}		% closed linear span
\DeclareMathOperator{\chull}{co}			 	% convex hull
\DeclareMathOperator{\grad}{\nabla}			% gradient
\DeclareMathOperator{\dvg}{\nabla\mdot}		% divergence
\DeclareMathOperator{\rot}{\nabla\times}		% curl
\DeclareMathOperator{\curl}{\rot}			% alternate
\DeclareMathOperator{\erf}{erf}				% error function
\DeclareMathOperator{\erfc}{erfc}			% complementary error function
\DeclareMathOperator{\esssup}{esssup}			% essential supremum


%%% Asymptotic notation

\DeclareMathOperator{\landauo}{\mathit{o}}
\DeclareMathOperator{\landauO}{\mathcal{O}}

\DeclareMathOperator{\landauTheta}{\Theta}
\DeclareMathOperator{\landauOmega}{\Omega}

%%%%%% General Math Macros %%%%%%%%%%%%%%
\safemath{\fun}{x}						% generic scalar function
\safemath{\altfun}{y}
\safemath{\aaltfun}{\sch}
\safemath{\bel}{\sce}					% basis element
\safemath{\altbel}{\sce}					% alternative basis element
\safemath{\frel}{g}					% frame element
\safemath{\altfrel}{g}					% alternative frame element
\safemath{\dfrel}{\tilde{g}}					% dual frame element
\safemath{\altdfrel}{\tilde{g}}					% alternative dual frame element

\safemath{\mat}{\matA}						% generic matrix
\safemath{\matc}{\matAc}						% components of a generic matrix
\safemath{\altmat}{\matB}						% alternative generic matrix
\safemath{\altmatc}{\matBc}						% alternative generic matrix


\safemath{\vectr}{\vecu}						% generic vector
\safemath{\vectrc}{\vecuc}						% components of a generic vector
\safemath{\altvectr}{\vecv}						% alternative generic vector
\safemath{\altvectrc}{\vecvc}						% components of an alternative generic vector

\newcommand{\nullspace}{\setN}	 			% nullspace
\newcommand{\rng}{\setR}		 				% range
\newcommand{\dom}{\setD}						% domain
\newcommand{\orth}{\perp}					% orthogonal
\newcommand{\simplifiedmathchoice}[2]{\mathchoice{#1}{#2}{#2}{#2}}

\newcommand{\Ex}[2]{\simplifiedmathchoice{\ensuremath{\Exop_{#1}\lefto[#2\right]}}{\ensuremath{\Exop_{#1}\bigl[#2\bigr]}}} 	% expectation
%\newcommand{\Var}[1]{\simplifiedmathchoice{\ensuremath{\Varop\lefto[#1\right]}}{\ensuremath{\Varop\bigl[#1\bigr]}}} % variance
\newcommand{\Cov}[1]{\ensuremath{\Covop\lefto[#1\right]}} % covariance
%\newcommand{\abs}[1]{\simplifiedmathchoice{\left\lvert#1\right\rvert}{\bigl\lvert#1\bigr\rvert}}		% absolute value
%\newcommand{\abs}[1]{\mathchoice{{\left\lvert#1\right\rvert}}{{\bigl\lvert#1\bigr\rvert}}{{\left\lvert#1\right\rvert}}{{\left\lvert#1\right\rvert}}}		% absolute value
%\newcommand{\abs}[1]{\left\lvert#1\right\rvert}		% absolute value

%\newcommand{\Ex}[2]{\ensuremath{\Exop_{#1}\lefto[#2\right]}} 	% expectation
%\newcommand{\Var}[1]{\ensuremath{\Varop\lefto[#1\right]}} % variance
%\newcommand{\Cov}[1]{\ensuremath{\Covop\lefto[#1\right]}} % covariance
%\newcommand{\abs}[1]{\left\lvert#1\right\rvert}		% absolute value
\newcommand{\card}[1]{\lvert#1\rvert}			% cardinality of a set
\newcommand{\comp}[1]{\ensuremath{#1^{c}}}	% set complement
\newcommand{\union}{\cup}					% set union
\newcommand{\Union}{\bigcup}
\newcommand{\intersect}{\cap}				% set intersection
\newcommand{\Intersect}{\bigcap}
\newcommand{\pset}[1]{\mathscr{P}(#1)} 		% power set
\newcommand{\ind}[1]{\chi_{#1}}				% indicator function
%\safemath{\interior}{\mathrm{Int}}			% interior of a set
%\newcommand{\domain}[1]{\mathscr{D}(#1)}	 	% domain of a mapping
\newcommand{\vecnorm}[1]{\lVert#1\rVert}		% vector norm
\newcommand{\frobnorm}[1]{\vecnorm{#1}_{\text{F}}}	% Frobenius norm
\newcommand{\opnorm}[1]{\lVert#1\rVert}		% operator norm
\newcommand{\conj}[1]{\ensuremath{#1^{*}}} 	% conjugate 		
\newcommand{\tp}[1]{\ensuremath{#1^{\mathsf{T}}}} 		% transpose
\newcommand{\dir}[1]{\ensuremath{\hat{#1}}} 		% transpose
\newcommand{\herm}[1]{\ensuremath{#1^{\mathsf{H}}}} 	% hermitian transpose (Hilbert adjoint) //modified by Christoph Bunte
\newcommand{\ad}[1]{\ensuremath{#1^{*}}} 		% adjoint operator
\newcommand{\inv}[1]{\ensuremath{#1^{-1}}} 	% inverse
\newcommand{\pinv}[1]{\ensuremath{#1^{\dagger}}} 	% Moore-Penrose pseudo-inverse
\newcommand{\sqm}[1]{\ensuremath{#1^{1/2}}}	% square-root operator
\newcommand{\opt}[1]{\ensuremath{#1^{\star}}} 	% optimum parameter
\newcommand{\est}[1]{\ensuremath{\hat{#1}\xspace}} 	% estimate
\newcommand{\west}[1]{\ensuremath{\widehat{#1}}} % estimate
\newcommand{\avg}[1]{\ensuremath{\bar{#1}}}
\safemath{\dirac}{\delta}					% Dirac delta
\safemath{\diracp}{\dirac(\time)}			% 	''	parametrized
\safemath{\krond}{\dirac}					% Kronecker delta
\safemath{\indfun}{I}						% Indicator function
\safemath{\stepfun}{u}						% step function at zero

\newcommand{\allz}[2]{\ensuremath{#1=0,1,\ldots,#2-1}}% all definition by Moritz
\newcommand{\allzinf}[1]{\ensuremath{#1=0,1,\ldots}}% all definition by Moritz
\newcommand{\allo}[2]{\ensuremath{#1=1,2,\ldots,#2}}% all definition by Moritz
\newcommand{\seq}[1]{\left\{#1\right\}}		 % generic sequence
\newcommand{\seqi}[2]{\left\{#1\right\}_{#2}} % indexed sequence
\newcommand{\seqz}[3]{\left\{#1\right\}_{#2=0}^{#3-1}}% finite sequence
\newcommand{\sumz}[2]{\ensuremath{\sum_{#1=0}^{#2-1}}}
\newcommand{\sumo}[2]{\ensuremath{\sum_{#1=1}^{#2}}}
\newcommand{\suminf}[1]{\ensuremath{\sum_{#1=-\infty}^{\infty}}}
\newcommand{\sumzinf}[1]{\ensuremath{\sum_{#1=0}^{\infty}}}
\newcommand{\sumoinf}[1]{\ensuremath{\sum_{#1=1}^{\infty}}}
\newcommand{\prodz}[2]{\ensuremath{\prod_{#1=0}^{#2-1}}}
\newcommand{\prodo}[2]{\ensuremath{\prod_{#1=1}^{#2}}}
\newcommand{\infint}[2]{\int\limits_{#2}#1 d#2}	% indefinite integral
\newcommand{\infiint}[3]{\iint\limits_{#3\,#2}#1 d#2d#3} 	% ind. double integral
\newcommand{\fourint}[3]{\infint{#1\cexn{#3 #2}}{#2}}		% Fourier integral
\newcommand{\fourintinv}[3]{\infint{#1\cex{#3 #2}}{#2}}	% inv. Four. integral
\newcommand{\logdet}[1]{\log \det\lefto(#1\right)} % log det function
%\newcommand{\set}[1]{\left\{#1\right\}}		% set notation
\newcommand{\clos}[1]{\overline{#1}}			% set closure
\newcommand{\besselI}[1]{I_{#1}}				% mod. Bessel fun. first kind
\safemath{\upto}{\uparrow}
\safemath{\downto}{\downarrow}
\safemath{\iu}{\mathrm{i}}							% imaginary unit
\safemath{\maj}{\succ}
\newcommand{\essup}[1]{\ensuremath{\mathrm{ess}_{#1}\sup}}	% essential supremum
\newcommand{\elementof}[2]{\left[#1\right]_{#2}}		% element of a matrix
\newcommand{\elementofseq}[2]{\left(#1\right)_{#2}}		% element of a sequance 
%\newcommand{\imat}[1]{\matI_{#1}}			% identity matrix
\newcommand{\zmat}[1]{\matzero_{#1}}			% all-zero matrix
\newcommand{\dftmat}[1]{\matF_{#1}}			% DFT matrix
\newcommand{\diagd}[1]{\matD(#1)}               % diagonalized matrix
\safemath{\mdft}{\dftmat{}}					% 	''
\newcommand{\vdft}[1]{\vecf_{#1}}			% column of the DFT matrix
\safemath{\runity}{\beta}					% root of unity
\safemath{\eval}{\lambda}					% eigenvalue
\newcommand{\eigmax}[1]{\eval_{\max}(#1)}
\safemath{\veval}{\veclambda}				% eigenvalue vector
\newcommand{\cex}[1]{e^{\iu2\pi #1}}			% positive complex exponential
\newcommand{\cexn}[1]{e^{-\iu2\pi #1}}		% negative complex exponential
\safemath{\littleo}{\sco}					% Landau\s little o

\let\im\undefined
\safemath{\re}{\Re}				% real part
\safemath{\im}{\Im}				% imaginary part
\newcommand{\rep}[1]{\Re\{#1\}} 			% real part parametrized
\newcommand{\imp}[1]{\Im\{#1\}}			% imaginary part parametrized


%%%%%%% Symbols for Special Spaces %%%%%%%%%%
\safemath{\euclidspace}{\complexset}			% Euclidean space
\safemath{\confunspace}{\setC}				% space of continuous functions
\newcommand{\banachseqspace}[1]{l^{#1}}		% Banach sequence space
\safemath{\hilseqspace}{\banachseqspace{2}}	% Hilbert sequence space
\newcommand{\banachfunspace}[1]{\setL^{#1}}	% Banach function space
\safemath{\hilfunspace}{\banachfunspace{2}}	% Hilbert function space
\safemath{\hilfunspacep}{\hilfunspace(\complexset)}	% Hilbert function space parametrized
\newcommand{\hardyspace}[1]{\setH^{#1}}		% Hardy space
\safemath{\schwarzspace}{\setS}				% Schwarz space

\newcommand{\hadj}[1]{#1^{\star}}			% Hilbert adjoint operator

%%%%%% Special Symbols for Communications %%%%%%%
%\safemath{\SNR}{\text{\sc snr}} 				% signal to noise ratio
\safemath{\SNR}{\text{\sc snr}} 				% signal to noise ratio
\safemath{\SINR}{\text{\sc sinr}} 				% signal to interference plus noise ratio
\safemath{\No}{N_0}							% noise spectral density
\safemath{\Es}{E_s}							% energy per symbol
\safemath{\Eb}{E_b}							% energy per bit
\safemath{\EbNo}{\frac{\Eb}{\No}}
\safemath{\EsNo}{\frac{\Es}{\No}}
\safemath{\NoVar}{\variance}                 % noise variance

% Time-frequency notation
\let\time\undefined
\safemath{\time}{\sct}						% continuous time
\safemath{\dtime}{\sck}						% discrete time
\safemath{\delay}{\sctau}					% continuous delay
\safemath{\ddelay}{\scl}						% discrete delay
\safemath{\doppler}{\scnu}					% continuous doppler
\safemath{\ddoppler}{\scm}					% discrete doppler
\safemath{\freq}{\scf}						% frequency
\safemath{\dfreq}{\scn}						% discrete frequency
\safemath{\Dtime}{\Delta\time}
\safemath{\Dfreq}{\Delta\freq}
\safemath{\Ddtime}{\dtime}
\safemath{\Ddfreq}{\dfreq}
\safemath{\bandwidth}{\scB}
\safemath{\maxdoppler}{\doppler_{0}}			% maximum Doppler shift
\safemath{\maxdelay}{\delay_{0}}				% maximum delay
\safemath{\spread}{\Delta_{\CHop}}			% total channel spread
\DeclareMathOperator{\CHop}{\ensuremath{\opH}} % channel operator
%\safemath{\kernel}{\rndk_{\CHop}}			% operator kernel
\safemath{\kernelp}{\kernel(\time,\time')}	% 	''	parametrized
\safemath{\tvir}{\rndh_{\CHop}}				% time-varying impulse response
\safemath{\tvirp}{\tvir(\time,\delay)}		%	''	parametrized
\safemath{\tvirc}{\conj{\rndh}_{\CHop}}		% 	''	parametrized
\safemath{\tvtf}{\rndl_{\CHop}}				% time-varying transfer function
\safemath{\tvtfp}{\tvtf(\time,\freq)}			%	''	parametrized
\safemath{\tvtfc}{\conj{\rndl}_{\CHop}}		%	''	parametrized
\safemath{\spf}{\rnds_{\CHop}}				% spreading function
\safemath{\spfp}{\spf(\doppler,\delay)}		%	''	parametrized
\safemath{\spfc}{\conj{\rnds}_{\CHop}}		%	''	parametrized
\safemath{\bff}{\rndb_{\CHop}}				% bi-freuqency function
\safemath{\bffp}{\bff(\doppler,\freq)}		%	''	parametrized

% WSSUS correlation functions
\safemath{\irc}{\scr_{\rndh}}				% impulse response correlation fn.
\safemath{\tfc}{\scr_{\rndl}}				% time-frequency correlation fn.
\safemath{\spc}{\scr_{\rnds}}				% spreading fn. correlation fn.
\safemath{\bfc}{\scr_{\rndb}}				% bi-frequency correlation fn.

\safemath{\scaf}{\scc_{\rnds}}				% scattering function
\safemath{\scafp}{\scaf(\doppler,\delay)}		% 	''	parametrized
\safemath{\ccf}{\scc_{\rndl}}				% WSSUS tvtf correlation
\safemath{\ccfp}{\ccf(\Dtime,\Dfreq)}			% 	''	parametrized
\safemath{\cic}{\scc_{\rndh}}				% WSSUS tvir correlation
\safemath{\cicp}{\cic(\Dtime,\delay)}			% 	''	parametrized


\safemath{\mi}{\scI}							% mutual information
\safemath{\capacity}{\scC}					% capacity



%%%%%% probability theory stuff %%%%%%
\DeclareMathOperator{\Prob}{\opP}		% probability of an event
\newcommand{\pdf}[1]{\scf_{#1}}			% probability density function
\newcommand{\altpdf}[1]{\scg_{#1}}		% alternative pdf
\newcommand{\pmf}[1]{\scf_{#1}}			% probability mass function
\newcommand{\altpmf}[1]{\scg_{#1}}		% alternative pmf
\newcommand{\cdf}[1]{\scF_{#1}} 		% probability distribution function
\newcommand{\altcdf}[1]{\scG_{#1}}		% alternative cdf
\newcommand{\esd}[2]{\scF_{#1}^{#2}} 	% eigenvalue spectrum distribution
\newcommand{\aesd}[1]{\scF_{#1}} 		% asymptotic eigenvalue spectrum distribution
\newcommand{\aesdf}[1]{\scf_{#1}} 		% asymptotic eigenvalue spectrum density function
\newcommand{\stielt}[1]{G_{#1}} 		% Stieltjes transform


\newcommand{\mgf}[1]{M_{#1}}			% moment generating function
\newcommand{\entropy}{\scH}				% entropy
\newcommand{\diffent}{\mathsf{h}}				% differential entropy
\newcommand{\relent}[2]{\scD(#1\,||\,#2)} % relative entropy
\safemath{\normal}{\mathcal{N}}			% normal distribution
\safemath{\jpg}{\mathcal{CN}}			% jointly proper Gaussian
\safemath{\uniform}{\mathcal{U}}				% uniform distribution
\safemath{\mchain}{\leftrightarrow}		% Markov chain
\newcommand{\chisq}[1]{\chi_{#1}}		% Chi-square RV
\newcommand{\given}{\,\vert\,}				% conditioning
\newcommand{\setgiven}{\,\middle|\,}				% conditioning
\newcommand{\AIC}{\ensuremath{\mathrm{AIC}}} % Akaike's Information Criterion
\newcommand{\AICC}{\ensuremath{\mathrm{AICC}}} 

%%%%% Unit Denominators %%%%%%%%%%
\safemath{\dB}{\,\mathrm{dB}}
\safemath{\dBm}{\,\mathrm{dBm}}
\safemath{\Hz}{\,\mathrm{Hz}}
\safemath{\kHz}{\,\mathrm{kHz}}
\safemath{\MHz}{\,\mathrm{MHz}}
\safemath{\GHz}{\,\mathrm{GHz}}
\safemath{\s}{\,\mathrm{s}}
\safemath{\ms}{\,\mathrm{ms}}
\safemath{\mus}{\,\mathrm{\text{\textmu}s}}
\safemath{\ns}{\,\mathrm{ns}}
\safemath{\ps}{\,\mathrm{ps}}
\safemath{\meter}{\,\mathrm{m}}
\safemath{\mm}{\,\mathrm{mm}}
\safemath{\cm}{\,\mathrm{cm}}
\safemath{\m}{\,\mathrm{m}}
\safemath{\W}{\,\mathrm{W}}
\safemath{\mW}{\, \mathrm{mW}}
\safemath{\J}{\,\mathrm{J}}
\safemath{\K}{\,\mathrm{K}}
\safemath{\bit}{\,\mathrm{bit}}
\safemath{\nat}{\,\mathrm{nat}}

%%%%% Binary Relations %%%%%

\safemath{\define}{\triangleq}					% definition
\newcommand{\sameev}{\stackrel{\scriptscriptstyle{\lambda}}{\equiv}}
\newcommand{\sothat}{\,:\,}				% set notation
\newcommand{\composition}{\circ}			% composition of mappings
\providecommand{\inner}[2]{\ensuremath{\left\langle#1,#2\right\rangle}}% inner product <.,.>
\safemath{\equivalent}{\sim}
\safemath{\distas}{\sim}					% distributed according to
%\newcommand{\AND}{\,\mathbf{and}\,}		% logical AND
\newcommand{\OR}{\,\mathbf{or}\,}		% logical OR
\safemath{\sdiff}{\Delta}				% symmetric set difference
\safemath{\setdiff}{\setminus}				% set difference



% Number sets
\safemath{\reals}{\mathbb R}
\safemath{\positivereals}{\reals^{+}}
\safemath{\integers}{\mathbb Z}
\safemath{\posint}{\integers^{+}}
\safemath{\naturals}{\mathbb N}
\safemath{\posnaturals}{\naturals^{+}}
\safemath{\complexset}{\mathbb C}
\safemath{\rationals}{\mathbb Q}

\newcommand{\natseg}[2]{[#1 \text{\phantom{\tiny{.}}:\phantom{\tiny{.}}} #2]} % segment of natural numbers
\newcommand{\innatseg}[3]{#1\elem[#2\!:\!#3]} % number belongs to a segment of natural numbers
\newcommand{\matsegwb}[3]{\left[#1\right]_{\{ #2 , #3 \}}} % entry of a matrix or a vector
\newcommand{\vecsegwb}[2]{\left[#1\right]_{\{ #2 \}}} % entry of a matrix or a vector
\newcommand{\matseg}[3]{\left[#1\right]_{ #2 , #3 }} % entry of a matrix or a vector
\newcommand{\vecseg}[2]{#1_{ #2}} % entry of a matrix or a vector
%\newcommand{\natseg}[3]{#1\in[#2\!:\!#3]} % entry of a matrix or a vector


%functional analysis
\safemath{\iSet}{\setI}
\newcommand{\pSet}[1]{\colP(#1)}			% power set
\newcommand{\cprod}{\times}				% cartesian product
\safemath{\rel}{\bowtie}					% relation
\safemath{\eqrel}{\sim}					% equivalence relation
\safemath{\rlord}{\leq}					% reflexive linear ordering
\safemath{\slord}{<}						% strict linear ordering
\safemath{\rpord}{\preceq}				% reflexive partial ordering
\safemath{\rrpord}{\succeq}				% reversed reflexive partial ordering
\safemath{\spord}{\prec}					% strict partial ordering
\safemath{\sig}{\sigma}					% sigma-{algebra, ring,...}
\safemath{\metric}{d}					% metric
\newcommand{\oball}[2]{\setB_{#2}(#1)}	% open ball
\newcommand{\salgebra}{\sig-algebra\xspace}
\safemath{\setfun}{\Phi}					% set function
\safemath{\measure}{\mu}					% measure
\safemath{\altmeasure}{\lambda}					% measure
\newcommand{\almev}{\text{ a.e. }}				% almost everywhere
\newcommand{\outerm}[1]{#1^{\star}}		% marks outer measures.
\newcommand{\innerm}[1]{#1_{\star}}		% marks inner measures.
\safemath{\omeasure}{\outerm{\measure}}		% outer measure
\safemath{\imeasure}{\innerm{\measure}}		% inner measure	
\safemath{\aecol}{\colS^{\star}_{\measure}} % collection of almost equal sets
\safemath{\emeasure}{\bar{\measure}_{0}}	% measure extension
\safemath{\rmeasure}{\tilde{\measure}}	% restricted measure
\safemath{\bmeasure}{\measure_{0}}		% basic measure on a semiring
\safemath{\glength}{\measure_{\altfun}}	% generalized length
\safemath{\lebmea}{\lambda}				% Lebesgue length and measure
\safemath{\blebmea}{\lebmea_{0}}			% pre-lebesgue-measure
\newcommand{\pospart}[1]{#1^{+}}			% positive part of a function
\newcommand{\negpart}[1]{#1^{-}}			% negative part of a function
\safemath{\sfun}{s}						% simple function
\safemath{\absintspace}{\colL^{1}}		% space of abs. integrable functions
\safemath{\sqintspace}{\banachfunspace{2}}		% space of square integrable functions
\safemath{\abssumspace}{l^{1}}		% space of abs. summable sequences
\safemath{\sqsumspace}{l^{2}}		% space of square summable sequences

\safemath{\sfield}{\setF}				% scalar field
\safemath{\vectors}{\setV}				% set of vectors
\safemath{\vecspace}{(\vectors,\sfield)}	% vector space
\safemath{\linspace}{\setV}				% linear space
\safemath{\clinspace}{(\linspace,\sfield)} % linear space
\safemath{\nspace}{\setU}				% normed space
\safemath{\metspace}{\setM}				% metric space
\safemath{\bspace}{\setB}				% Banach space
\safemath{\ipspace}{\setG}				% inner product space
\safemath{\hilspace}{\setH}				% Hilbert space
\safemath{\blospace}{\setG}				% set of bounded linear oprators
\safemath{\lop}{\opT}					% linear operator
\safemath{\altlop}{\opS}					% alternative linear operator
\safemath{\nullsp}{\nullspace(\lop)}		% null space of the linear operator
\safemath{\lfun}{l}						% linear functional
\safemath{\altlfun}{g}					% alternative linear functional
\newcommand{\adual}[1]{#1^{\star}}		% algebraic dual space
\newcommand{\dual}[1]{#1^{'}}			% dual space
\newcommand{\ocomp}[1]{#1^{\orth}}		% orthogonal complement
\safemath{\dsum}{\oplus}					% direct sum
\safemath{\funspace}{\colL}				% function space
\renewcommand{\adj}[1]{#1^{\times}}		% adjoint operator generator
\safemath{\adjlop}{\adj{\lop}}			% adjoint operator
%\newcommand{\hadj}[1]{#1^{\star}}		% Hilbert adjoint operator generator
\safemath{\hadjlop}{\hadj{\lop}}			% Hilbert adjoint operator
\safemath{\tow}{\xrightarrow{w}}			% weak convergence
\safemath{\tows}{\xrightarrow{w^{*}}}		% weak* convergence
\safemath{\cparam}{\lambda}
\safemath{\lopl}{\lop_{\cparam}}		
\safemath{\iop}{\opI}					% identity operator
\safemath{\resolop}{\opR}				% resolvent operator
\safemath{\resolvent}{\resolop_{\cparam}(\lop)}	% resolvent operator
\safemath{\reset}{\setQ}
\safemath{\spectrum}{\setS}
\safemath{\resolset}{\reset(\lop)}		% resolvent set
\safemath{\lopspec}{\spectrum(\lop)}		% spectrum of a linear operator
\safemath{\pspec}{\spectrum_{p}(\lop)}	% point spectrum
\safemath{\cspec}{\spectrum_{c}(\lop)}	% continuous spectrum
\safemath{\rspec}{\spectrum_{r}(\lop)}	% residual spectrum
%\safemath{\ev}{\cparam}					% eigenvalue
\newcommand{\specrad}[1]{r_{#1}}			% spectral radius
\safemath{\lopsrad}{\specrad{\lop}}		% spectral radius
\safemath{\pop}{\opP}					% projection operator
\newcommand{\restrict}[2]{#1\rvert_{#2}}
\safemath{\specfam}{\colE}				% spectral family
\safemath{\specop}{\opE_{\cparam}}		% spectral projection operator
\safemath{\altspecop}{\opE_{\mu}}		% alternat spectral projection operator
\newcommand{\rlim}[1]{#1^{+}}			% right limit
\newcommand{\llim}[1]{#1^{-}}			% left limit
\safemath{\vmulti}{\vecone}				% vector multiplicative identity
\newcommand{\hsnorm}[1]{\opnorm{#1}\sub{HS}}	% Hilbert-Schmidt norm
%\safemath{\hilfunspace}{\funspace^{2}}	% Hilbert function space
%\safemath{\kernel}{k}					% integral kernel
\safemath{\unitaryop}{\opU}				% unitary operator
\safemath{\sval}{\sigma}					% singular value
\newcommand{\trnorm}[1]{\opnorm{#1}\sub{tr}}	% trace norm
\safemath{\corrcoef}{\rho}				% canonical correlation coefficient
\safemath{\sangle}{\theta}				% angle between subspaces

%frames
\let\time\undefined
\safemath{\iset}{\setI}				% index set
\safemath{\shift}{\nu}
\safemath{\scale}{\alpha}
\safemath{\time}{t}
\safemath{\specfreq}{\theta}	
\newcommand{\transopgen}[1]{\opT_{#1}} % translation operator
\safemath{\transop}{\transopgen{\delay}}
\newcommand{\modopgen}[1]{\opM_{#1}}	% modulation operator
\safemath{\modop}{\modopgen{\shift}}
\newcommand{\dilopgen}[1]{\opD_{#1}}	% dilation operator
\safemath{\dilop}{\dilopgen{\scale}}
\newcommand{\dualspace}[1]{#1^{'}}	% dual space
\safemath{\fram}{\setF}				% frame
\safemath{\dfram}{\dual{\fram}}		% dual frame
\safemath{\ufb}{B}					% upper frame bound
\safemath{\lfb}{A}					% lower frame bound
\safemath{\sop}{\hadj{\aop}}				% frame synthesis operator
\safemath{\aop}{\opT}			% frame analysis operator 		// modifide by christoph bunte
\safemath{\fop}{\opS}				% frame operator 			// modified by christoph bunte 
\safemath{\daop}{\tilde\opT}			% dual frame analysis operator 		// added by christoph bunte
\safemath{\dsop}{\hadj{\tilde\opT}}				% dual frame synthesis operator 			// added by christoph bunte 

\safemath{\ifop}{\inv{\fop}}			% inverse frame operator
\safemath{\rifop}{\fop^{-1/2}}			% square root of inverse frame operator
\newcommand{\ft}[1]{\widehat{#1}}	% Fourier transform
\newcommand{\ftd}[1]{\widehat{#1}_d}	% Fourier transform
\safemath{\transeq}{\setT}			% sequence of translates
\safemath{\nfun}{\Phi}				% ``Nyquist series''
\safemath{\funvec}{\vecf}			%  function as a vector
\safemath{\altfunvec}{\vecg}

%probability
\safemath{\samplespace}{\Omega}
\safemath{\probspace}{(\samplespace,\sfield,\Prob)}	% probability space
\safemath{\ccoef}{\rho}			% correlation coefficient
% discrete-time random processes of infinite duration
\newcommand{\dtrandproc}[1]{\{X_{#1}\}_{#1=1}^{\infty}}
\newcommand{\altdtrandproc}[1]{\{Y_{#1}\}_{#1=1}^{\infty}}
% Markov chain stuff
\newcommand{\nstep}[2]{P_{#1}^{(#2)}}		% n-step transition probability
\newcommand{\bnstep}[1]{\bP^{#1}}		% n-step transition probability matrix
%\newcommand{\acc}{\rightarrow}			% accessible states
\newcommand{\com}{\leftrightarrow}		% communicating states
\newcommand{\per}[1]{d(#1)}				% period of an MC
\newcommand{\nstate}[1]{\vecpi^{(#1)}}	% state vector
\safemath{\infstate}{\vecpi}				% steady state vector
\safemath{\typset}{\setA_{\epsilon}^{(N)}}	% typical set
\safemath{\expequal}{\doteq}				% equal to first order in the exponent
\safemath{\code}{C}						% code
\safemath{\dstringset}{\setD^{\star}}		% set of finite length D-ary strings
\safemath{\cwlength}{l}					% codeword length
\safemath{\elength}{L}					% expected codeword length
\safemath{\extension}{C^{\star}}			% code extension
\safemath{\approaches}{\rightarrow}		% i.e., x_{n} -> x
\safemath{\evnt}{\setA}					% event A
\safemath{\altevnt}{\setB}					% event B
%\safemath{\rv}{\rndx}					% random variable X
\safemath{\altrv}{\rndy}					% random variable Y
\safemath{\complexrv}{\rndu}					% complex random variable U
\safemath{\altcrv}{\rndv}				% complex random variable V
\safemath{\rvec}{\rvecx}					% random vector X
\safemath{\altrvec}{\rvecy}				% random vector Y
\safemath{\crvec}{\rvecu}				% complex random vector U
\safemath{\altcrvec}{\rvecv}				% complex random vector V
\newcommand{\ifunc}[1]{I_{#1}}			% indicator function
\newcommand{\moment}[1]{m_{#1}}			% higher-order moment
%\newcommand{\mean}[1]{\mu_{#1}}			% scalar mean
\newcommand{\mvec}[1]{\vecmu_{#1}}		% mean vector
\newcommand{\cmoment}[1]{\sigma_{#1}}		% higher-order central moment
%\safemath{\variance}{\sigma^{2}}			% variance
\newcommand{\rp}[1]{#1_{R}}				% real part
\newcommand{\ip}[1]{#1_{I}}				% imaginary part
\newcommand{\rcc}[1]{\widetilde{#1}}		% complex extension
\newcommand{\covmat}[1]{\matK_{#1}}		% covariance matrix
\newcommand{\pcovmat}[1]{\matJ_{#1}}		% pseudocovariance matrix
\safemath{\map}{T}						% mapping
\safemath{\jacobian}{J}					% jacobian
\newcommand{\cormat}[1]{\matR_{#1}}		% correlation matrix
%mylatex
\safemath{\wvec}{\rvecw}					% white random vector
\safemath{\wrv}{\rndw}					% white noise process
\safemath{\orthmat}{\matQ}				% orthogonal matrix
\safemath{\evmat}{\matLambda}			% eigenvalue matrix (diagonal)
\safemath{\identity}{\matidentity}		% identity matrix
\safemath{\innovec}{\vecv}				% innovations vector
\safemath{\convas}{\xrightarrow{\text{a.s.}}}	% almost sure convergence
\safemath{\convr}{\xrightarrow{\text{r}}}	% convergence in r-th mean
\safemath{\convp}{\xrightarrow{\text{P}}}	% convergence in probability
\safemath{\convd}{\xrightarrow{\text{D}}}	% convergence in distribution
\newcommand{\corf}[1]{R_{#1}}		% correlation function
\newcommand{\covf}[1]{K_{#1}}		% covariance function
\newcommand{\pcovf}[1]{J_{#1}}		% pseudocovariance function
\newcommand{\psd}[1]{S_{#1}}			% power spectral density
\safemath{\ltis}{\opL}				% LTI system
\safemath{\ir}{h}					% impulse response
\safemath{\tf}{\MakeUppercase{\ir}}	% transfer function
\newcommand{\chf}[1]{\Phi_{#1}}		% characteristic function


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %: theorems, lemmata, etc.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% definitions for the fancyref  package
% prefixes
\newcommand*{\fancyrefparlabelprefix}{par}		% Part
\newcommand*{\fancyrefchalabelprefix}{cha}		% Chapter
\newcommand*{\fancyrefapplabelprefix}{app}		% Appendix
\newcommand*{\fancyrefthmlabelprefix}{thm}		% Theorem
\newcommand*{\fancyreflemlabelprefix}{lem}		% Lemma
\newcommand*{\fancyrefcorlabelprefix}{cor}		% Corolary
\newcommand*{\fancyrefdeflabelprefix}{dfn}		% Definition
\newcommand*{\fancyrefproplabelprefix}{prop}		% Property
\newcommand*{\fancyrefexlabelprefix}{ex}		% Example
\newcommand*{\fancyrefxcalabelprefix}{xca}		% Exercise

% label names
\frefformat{vario}{\fancyrefparlabelprefix}{Part~#1}
\frefformat{vario}{\fancyrefchalabelprefix}{Chapter~#1}
\frefformat{vario}{\fancyrefseclabelprefix}{Section~#1}
\frefformat{vario}{\fancyrefthmlabelprefix}{Theorem~#1}
\frefformat{vario}{\fancyreflemlabelprefix}{Lemma~#1}
\frefformat{vario}{\fancyrefcorlabelprefix}{Corollary~#1}
\frefformat{vario}{\fancyrefdeflabelprefix}{Definition~#1}
\frefformat{vario}{\fancyreffiglabelprefix}{Figure~#1}
\frefformat{vario}{\fancyrefapplabelprefix}{Appendix~#1}
\frefformat{vario}{\fancyrefeqlabelprefix}{(#1)}
\frefformat{vario}{\fancyrefproplabelprefix}{Property~#1}
\frefformat{vario}{\fancyrefexlabelprefix}{Example~#1}
\frefformat{vario}{\fancyrefxcalabelprefix}{Exercise~#1}

% theorems, lemmata, etc.
%--
% \theoremstyle{plain}
% \newtheorem{thm}{Theorem}
%\newtheorem{example}[thm]{Example}
%\newtheorem{prop}{Property}


%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  abriviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\iid}{i.i.d.\@\xspace}
\newcommand{\as}{a.s.\@\xspace}
\newcommand{\wrt}{w.r.t.\@\xspace}



